Multi-Sem Fusion: Multimodal Semantic Fusion for 3D Object Detection

LiDAR and camera fusion techniques are promising for achieving 3D object detection in autonomous driving. Most multi-modal 3D object detection frameworks integrate semantic knowledge from 2D images into 3D LiDAR point clouds to enhance detection accuracy. Nevertheless, the restricted resolution of 2D feature maps impedes accurate re-projection and often induces a pronounced boundary-blurring effect, which is primarily attributed to erroneous semantic segmentation. To well handle this limitation, we propose a general multi-modal fusion framework Multi-Sem Fusion (MSF) to fuse the semantic information from both the 2D image and 3D points scene parsing results. Specifically, we employ 2D/3D semantic segmentation methods to generate the parsing results for 2D images and 3D point clouds. The 2D semantic information is further reprojected into the 3D point clouds with calibration parameters. To handle the misalignment between the 2D and 3D parsing results, we propose an Adaptive Attention-based Fusion (AAF) module to fuse them by learning an adaptive fusion score. Then the point cloud with the fused semantic label is sent to the following 3D object detectors. Furthermore, we propose a Deep Feature Fusion (DFF) module to aggregate deep features at different levels to boost the final detection performance. The effectiveness of the framework has been verified on two public large-scale 3D object detection benchmarks by comparing them with different baselines. The experimental results show that the proposed fusion strategies can significantly improve the detection performance compared to the methods using only point clouds and the methods using only 2D semantic information. Most importantly, the proposed approach significantly outperforms other approaches and sets state-of-the-art results on the nuScenes testing benchmark.

==> Files/01_introduction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}\label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\IEEEPARstart{P}{erception} of obstacles' 3D information via different types of sensors is a fundamental task in the field of computer vision and robotics. This topic has been extensively studied with the development of Autonomous Driving(AD) and intelligent transportation system. We can easily get distance information of the obstacles from LiDAR sensors, and the texture and color information has been totally lost due to the sparse scanning. Therefore, False Positive (FP) detection and wrong categories classification often happen for LiDAR-based object detection frameworks. In particular, with the development of the deep learning techniques on point-cloud-based representation, {LIDAR-based approaches} can be generally divided into point-based \cite{shi2019pointrcnn}, voxel-based \cite{zhou2018voxelnet, lang2019pointpillars,yan2018second}, and hybrid-point-voxel-based methods \cite{shi2020pv}.

\begin{figure}[t!]
	\centering
	\includegraphics[width=0.45\textwidth]{Figs/Head_chart.pdf}
	\centering
	\caption{The proposed \textit{Multi-Sem Fusion (MSF)} is a general multi-modal fusion framework which can be employed for different 3D object detectors. a) illustrate the improvements on three different baselines. b) gives the performance of \textit{CenterPoint} \cite{yin2021center} with the proposed modules on the public nuScenes benchmark. c) gives the improvements on different categories respectively. In addition, ``w/o'' represent ``without'' in short.}  
	\label{Fig:head_figure}
\end{figure}

On the other hand, the sensor of cameras can provide details texture and color information while the distance information has been totally lost. %\during the perspective projection process. xsqcomments{likes humans see. However, in general, depth information measured by camera is not accurate}.
The fusion method with various sensor data is an encouraging way for boosting the perception performance of AD. Generally, multi-modal fusion approaches in object detection tasks can be divided into early fusion-based \cite{dou2019seg, vora2020pointpainting}, deep fusion-based \cite{zhang2020maff, xu2018pointfusion, tian2020adaptive} and late fusion-based approaches \cite{pang2020clocs}. Early fusion-based approaches aim to create a new type of data by directly combining the raw data before inputting it into the detection framework. Typically, such methods require pixel-level correspondence between different sensor data types. Different from the early fusion-based methods, late fusion-based approaches {fuse the detection results at the bounding box level. While} deep fusion-based methods usually extract the features with different types of deep neural networks first and then fuse them at the features level.  {\textit{PointPainting} \cite{vora2020pointpainting} is an early fusion method which} achieves superior detection results on different benchmarks. {Specifically, The network takes point clouds together with the 2D image semantic predictions as inputs and output the detection results with any LiDAR-based 3D object detector.} {More importantly, it} can be incorporated into any 3D object detectors {regardless of} point-based or voxel-based frameworks.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.45\textwidth]{Figs/head.pdf}
	\centering
	\caption{(a) shows the point cloud with the 2D segmentation results, where the frustum within the blue line highlight indicates misclassified areas due to the blurring effect at the object's boundary; (b) displays the 3D segmentation results, where misclassified points are colored in red; (c) and (d) show the results based on 2D painted point cloud (with an obvious False Positive (FP) Detection) and the proposed \textit{Multi-Sem Fusion (MSF)} framework respectively.} %The boundary blurring effect in the image-based semantic segmentation results
	\label{Fig:2DSeg_in_3d}
\end{figure}

However, the {blurring effect at object's boundary} often happens inevitably in image-based semantic segmentation methods. This effect becomes much worse when reprojecting the 2D semantic projections into the 3D point clouds. An example of this effect has been shown in Fig. \ref{Fig:2DSeg_in_3d}. Taking the big truck at the left bottom of the sub-fig. An instance of this issue is illustrated in \ref{Fig:2DSeg_in_3d}-(a), the significant frustum area in the blue line highlight of the background (i.e., orange points) incorrectly classified as foreground due to inaccurate projection. Additionally, the re-projection of 3D points onto 2D image pixels is not a one-to-one process because of the digital quantization and many-to-one projection issues. Notably, segmentation results from the 3D point clouds (as seen in sub-fig. \ref{Fig:2DSeg_in_3d}-(b)) outperform the 2D image at obstacle boundaries. However, the category classification from 3D point clouds often yields worse results (as demonstrated by points in red) when compared to the 2D image, primarily due to the loss of detailed texture information in point clouds.

%. Each lidar point is projected into the output of an image semantic segmentationnetwork and the channel-wise activations are concatenatedto the intensity measurement of each lidar point. The concatenated (painted) lidar points can then be used in any lidar detection method, whether bird’s-eye view [11, 29, 21, 34, 30, 32] or front-view [12, 17]. PointPainting addresses the shortcomings of the previous fusion concepts: it does not add any restrictions on the 3D detection architecture; it does not suffer from feature or depth blurring; it does not require a pseudo-point cloud to be computed, and it does not limit the maximum recall.

%Late fusion is more easier to build complete network,they even don't need incorporate pre-trained model,just associate at detection result in the end,and most deep fusion method adopted feature level fusion,it need reconstruct a new neural network.the motivation of Muti-modal is to make the accuracy be better,However,recently published LIDAR only method such as Second\cite{yan2018second}, PointRCNN\cite{shi2019pointrcnn},PV-RCNN\cite{shi2020pv},,CenterPoint\cite{yin2021center} has better performance than muti-sensor method, There a significant problem is that the relationship of point-to-pixel is not one-to-one,neighbored points into same pixel when we project point clouds to image,just like Fig.\ref{Fig:map_seg},we will get frustum points when we want get pixel information which associated with point. 

%With the advancement of technology and the continuous decline of lidar costs,3D Object detection has been got wide applications in various fields such as AD and kinds of robotics,and also a well-researched topic in academia.3D perception of vehicles and other objects needed  high accuracy in their environment, 2D visual perception usually has much texture information and higher resolution,it has obvious advantage in detect such as traffic light and lane,but 3D detection from point-Clouds provides more credible depth information,So LIDAR has great superiority in precise measurement of 3D position.

%According to the evaluation result on the challenging nuScenes vision benchmark\cite{nuScenesDetBenchmark},the best 3D detection method,PVC-ensemble,has achieved 65.2\% mean average precision (mAP),nuScenes detection score(NDS) 70.2\%  by LIDAR based only method,whereas the highest result of 3D object detection method,FOCOS3D,just got 35.8\% mean average precision(mAP),and nuScenes detection score(NDS) 42.8\% by pure Camera detect method ,There appear a large performance gap.Is this mean 2D vision perception is useless?The answer,as we all know,must be no negative, because the information we get from LIDAR and Camera is difference as above we discussed,deep learning has shown excellent performence both in object detection and segmentation filed,Camera has special advantages in precise classification,It has been widely used in recent years,one possible way is to take full advantage of the complementary information between camera and LIDAR.

%Just as the two example Shown in Fig. \ref{Fig:map_seg} 
%\begin{figure}[ht!]
%	\centering
%	\includegraphics[width=0.45\textwidth]{TITS/Figs/Mapseg.pdf}
%	\centering
%	\caption{FP and distance.}
%	\label{Fig:map_seg}
%\end{figure} where the outline of xx in the left lower  picture is very similar with car in 3D point cloud,it hard to distinguish the really type using only LIDAR,on other hand,because of characteristics of LIDAR,there has only few points in long distance,it also difficult to predict in this situation even missing the obstacles,But 2D image has rich texture information can easy identify witch type it belong to,Which is show that fusion both image and point cloud information is useful to help effectively reduce 3D false positive(FP) and increasing the object detection accuracy.

%Muti-modal detection methods can be divided into three classes, early fusion[\cite{dou2019seg},\cite{vora2020pointpainting}],deep fusion[\cite{zhang2020maff},\cite{xu2018pointfusion},\cite{tian2020adaptive}] and late fusion[\cite{pang2020clocs}],each with their own pluses and minuses,early fusion aim to create a new type data which combines diff sensors,typically require pixel-level correspondences of sensor data.Late fusion is more easier to build complete network,they even don't need incorporate pre-trained model,just associate at detection result in the end,and most deep fusion method adopted feature level fusion,it need reconstruct a new neural network.the motivation of Muti-modal is to make the accuracy be better,However,recently published LIDAR only method such as Second\cite{yan2018second}, PointRCNN\cite{shi2019pointrcnn},PV-RCNN\cite{shi2020pv},,CenterPoint\cite{yin2021center} has better performance than muti-sensor method, There a significant problem is that the relationship of point-to-pixel is not one-to-one,neighbored points into same pixel when we project point clouds to image,just like Fig.\ref{Fig:map_seg},we will get frustum points when we want get pixel information which associated with point.

The effectiveness of PointPainting, which utilizes 2D image semantic information for 3D object detection has been demonstrated despite some semantic errors. However, a natural question arises: can the final detection performance be further improved by fusing both the 2D and 3D semantic results in an effective way? To address this question, we introduce a general multi-modal fusion framework \textit{Multi-Seg Fusion} and fusion of diverse sensor data types at the semantic level to improve the final 3D object detection performance. First of all, {we obtain the 2D/3D semantic information throughout 2D/3D parsing approaches by taking images and raw point clouds.  Each point in point cloud has two types of semantic information after projecting point clouds onto 2D semantic images based on the intrinsic and extrinsic calibration parameters.}, the semantic results conflict usually happens for a certain point, rather than concatenating the two types of information directly, we propose an AAF strategy to fuse different kinds of semantic information in a point or voxel-level adaptive manner. This is achieved based on the learned context features with the self-attention mechanism. Specifically, an attention score has been learned for each point or vox el to balance the importance of the two different semantic results.
 
Furthermore, {in order to detect  obstacles with different sizes in an efficient way}, a DFF module is proposed here to fuse the features {at multi-scale receptive fields and a channel attention network to gather related channel information in the feature map}. Then the fused features are passed for the following classification and regression heads to generate the final detection. As the results on nuScenes dataset are given in \figref{Fig:head_figure} (a), we can obviously find that the proposed modules can robustly boost the detection performance on different baselines. {The results in \figref{Fig:head_figure}(b) illustrates the contribution of each module we proposed} and from this figure, it can be observed that the detection results can be consistently improved by adding more modules gradually. 
%is the results of original CenterPoint, CenterPoint-painting, FusionPainting \cite{xu2021fusionpainting} and our Multi-Sem Fusion, it shows a gradually increase and our method got best. 
\figref{Fig:head_figure} (c) shows the improvements on different categories and from this figure we can easily find that all the classes have been improved and ``Bicycle'' gets the most improvement (e.g., 22.3 points) on the nuScenes dataset.
 
%To further improve the performance, an attention module is proposed to fuse different kinds of semantic information in voxel-level adaptively based on the learned context features in a self-attention style. Finally, the points painted by the fused semantic labels are sent to 3D detectors for obtaining the final detection results. 
%In this papers,we propose a state of the art network called Adaptive-MutiSegFusionNet: a robust and accuracy early fusion muti-modal network use both 2D image and 3D points cloud  semantic segmentation information,the work is inspired by PointPaintinng\cite{vora2020pointpainting}, on hand,Each lidar point will project into 2D semantic segmentation mask image to get painted lidar point as describe in \cite{vora2020pointpainting},on another hand,raw point cloud as input data to a 3D semantic modal, there we got both 2D pixel level and 3D point level semantic feature,then sent them to adaptive weight learning network,aim to reduce the influence of frustum effect,in the view of that Adaptive-MutiSegFusionNet is First framework to adopt multi-semantic infos from both image and points cloud.and we argue that fusion extra semantic feature from muti sensor data is a effective way to get higher performance of 3D detector.

This manuscript extends a previously published conference paper \cite{xu2021fusionpainting} with new relevant state-of-the-art methods, theoretical developments, and experimental results. Compared to the previous conference paper, this work significantly improves the 3D object detection accuracy hugely on the nuScenes 3D object detection benchmark. Moreover, we also evaluate the proposed framework on the KITTT 3D object detection dataset, and the experimental results on both public datasets demonstrate the superiority of our framework. In generally, this work can be characterized by the following contributions: 
\begin{enumerate}
 \item %{A general multi-modal fusion framework  has been proposed to fuse the different types of sensors in the semantic level to boost the 3D object detection performances.}
 The proposed \textit{Multi-Sem Fusion} framework offers a general approach for multi-modal fusion that operates at the semantic level, which helps improve 3D object detection performance by integrating different types of sensors.
   \item Rather than combining different semantic results directly, an adaptive attention-based fusion module %{is proposed to fuse different kinds of semantic information in point or voxel-level by learning the fusion attention scores.}
   is introduced, which learns fusion attention scores instead of directly combining the results.
   \item Furthermore, a deep features fusion module is also proposed to fuse deep features at different levels to better detect objects of various sizes. This is achieved by fusing deep features extracted from different layers of the network and channel attention technology.
  \item Finally, the proposed framework has been sufficiently evaluated on two public large-scale 3D object detection benchmarks and the experimental results demonstrate the superiority of the proposed fusion framework. The proposed approach achieves SOTA results on the nuScenes dataset and outperforms other approaches with a big margin. Taking the proposed framework as the baseline, we have won the fourth nuScenes detection challenge held at ICRA 2021 on 3D Object Detection open track \footnote{\url{https://eval.ai/web/challenges/challenge-page/356/leaderboard/1012}}. 
\end{enumerate}






%The main contributions of this work can be summarized as following:
% \begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
%\begin{enumerate}
%   \item A general multi-modal fusion framework \textit{FusionPainting} has been firstly proposed to fuse the different types of information in the semantic level to improve the 3D object detection performance.
%   \item To further improve the performance, an attention module is proposed to fuse different kinds of semantic information in voxel-level by learning the context features. % this strategy can further improve results. 
  %First multi-modal framework to fusion both 3D points cloud and 2D image semantic information, the performance getting significantly improved.
%  \item The experimental results on the large-scale AD benchmark nuScenes show the superiority of the proposed fusion framework and achieve SOTA results compared to other methods. 
   %A weakly self-attention model used to learn the weight of 3D point-level semantic and 2D semantic pixel-level feature,and reduce the impact of frustum effect.
%\end{enumerate}








==> Files/02_related_work.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}\label{sec:related_work}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\ {We need give a more comprehensive survey of recently proposed multi-modal-fusion-based approaches.} 


% \begin{table*}[]
% \centering
% \resizebox{0.75\textwidth}{!}{
% \begin{tabular}{l|c|l}
%   \hline
%   \multicolumn{1}{c|}{\multirow{2}{*}{Multi-modal Fusion}} &
%   \multicolumn{1}{c|}{\multirow{2}{*}{Inputs}} &
%   \multicolumn{1}{c}{\multirow{2}{*}{Descriptions}} \\
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c|}{} &
%   \multicolumn{1}{c}{} \\ \hline
%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   \begin{tabular}[c]{@{}l@{}} Early Fusion  \end{tabular} & \\
%   \begin{tabular}[c]{@{}l@{}} Middle Fusion \end{tabular} & \\
%   \begin{tabular}[c]{@{}l@{}} Late Fusion  \end{tabular} & \\
%   \begin{tabular}[c]{@{}l@{}} Deep Fusion  \end{tabular} &
%   \\ \hline
%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   %\begin{tabular}[c]{@{}l@{}} tightly coupled  \end{tabular} &
%   %\begin{tabular}[c]{@{}l@{}} image  Lidar \end{tabular} &
%   %\begin{tabular}[c]{@{}l@{}} XX \end{tabular} \\ \hline
% \end{tabular}
% }
% \caption{\normalfont An overview of multi-modal-fusion-based 3D object detection approaches, including before, middle and after fusion, etc.}
% 	\label{tab:different_fusion_approaches}
% \end{table*}

Generally, 3D object detection methods can be categorized as LiDAR-based, image-based \cite{ku2019monocular} and multi-modal fusion-based, which takes LiDAR point cloud, image and multi-sensor captured data as inputs, respectively. 

\subsection{{LiDAR-based 3D Object Detection}}

The existing LIDAR-{based} 3D object detection methods {can be generally categorized into three main groups as} projection-based~\cite{ku2018joint,luo2018fast,yang2018pixor,liang2021rangeioudet,hu2020you}, voxel-based~\cite{zhou2018voxelnet,yan2018second,kuang2020voxel, yin2020lidar,zhou2019iou} and point-based~\cite{zhou2020joint,lang2019pointpillars,qi2018frustum}. 
RangeRCNN \cite{liang2021rangeioudet} proposed a 3D range {image-based} 3D object detection framework {where} the anchors could be generated on the BEV (bird’s-eye-view) map. VoxelNet \cite{zhou2018voxelnet} is the first {voxel-based} framework, which uses a VFE (voxel feature encoding) layer {to extract the point-level features for each voxel.} {To accelerate the inference speed,} SECOND \cite{yan2018second} presents a new framework which {employs} the sparse convolution \cite{graham20183d} to replace the heavy 3D convolution operation. {Inspired by the 2D anchor-free object detector CenterNet \cite{duan2019centernet}, CenterPoint \cite{yin2021center} presented an anchor-free approach for 3D object detection on LiDAR point clouds, and achieved SOTA (state-of-the-art) performance on the nuScenes benchmark recently. To further improve the efficiency,} PointPillars \cite{lang2019pointpillars} divides the points into vertical columns (e.g., pillars) and extracts features from each pillar with the PointNet \cite{qi2017pointnet} module. Then, the 2D feature map with the shape of $ {H*W*C}$ can be regarded as a pseudo image and all the 2D object detection pipelines to the feature map enable their use for 3D object detection. Different from the regular representation like voxel or pseudo image, {PointRCNN \cite{shi2019pointrcnn} directly extracts features from the raw points cloud and generates the proposals from the foreground points. Based on the PointRCNN, PV-RCNN \cite{shi2020pv} takes both the advantage from voxel and points representation and learns more discriminative features by employing both 3D voxel-based convolutional neural network and PointNet-based networks together.}
\subsection{{image-based 3D Object Detection}}
Stereo rigs \cite{zhou2014modeling} method can be used for 3D object detection by first detecting the 2D object from the image, and then recovering the distance using traditional geometric stereo matching techniques\cite{Efficient2010}. {Currently, with sufficient training data}, the depth can be recovered from a single image \cite{song2021mlda}. Generally, image-based 3D object detection methods that use deep learning can be divided into CAD Model-guided based, depth estimation-based and direct regression-based respectively. MANTA (Many-Tasks) \cite{chabot2017deep} is an image-based framework designed for many-task vehicle analysis. It is capable of simultaneously detecting vehicles, localizing parts, characterizing visibility, and estimating 3D dimensions, among other tasks. {In \cite{song2019apollocar3d}, a large-scale dataset ApolloCar3D is provided for instance-level 3D car understanding. Based on this dataset, a key-points-based framework has been designed by extracting the key points first, and then the vehicle pose is obtained using a PnP solver.} Furthermore, a {novel} work \cite{ku2019monocular} leverages {object} proposals and shapes reconstruction {through an end-to-end framework.} With the rapid development of single-image depth estimation technology, {leveraging} the depth information for 3D object detection becomes popular. \cite{wang2019pseudo} and \cite{qian2020end} {compute the disparity map from stereo image pair and} convert the depth maps to pseudo-LiDAR point clouds first. Then any 3D points cloud detectors can be employed for the 3D object detection task. The similar idea has been employed in \cite{weng2019monocular}, \cite{ma2019accurate} and \cite{cai2020monocular}. Instead of using CAD models or depth estimation, ``SMOKE'' \cite{liu2020smoke} proposes directly regressing the 3D bounding box from the image and achieving promising performance on the KITTI benchmark. Based on this, \cite{zhou2020iafa} proposes a plug-and-play module IAFA to aggregate useful foreground information in an instance-aware manner for further improving the detection accuracy.


\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.85\textwidth]{Figs/frame.pdf}
	\centering
	\caption{Overview of the proposed \textit{Multi-Sem Fusion} framework. We first obtain the semantic information from both input point clouds and 2D images with 2D and 3D parsing approaches. The semantic information from the two types of data is then fused at the semantic level using the proposed AAF module. Furthermore, a DFF module is also proposed to fuse the deep features at different spatial levels to boost the detection for accurate kinds of size object. Finally, fused features are sent to the detection heads for producing the final detection results.
}
	\label{Fig:PointPainting}
\end{figure*}






%for 3D LIDAR point-clouds representation, existing 3D object detection methods have explored several ways to achieved detection task,i.e.the Voxel-based mehtods and the point-based methods,Voxel-based methods like ,SECOND\cite{yan2018second} assume that  the environment is represented in a 3D grid,or a voxel representation,First build  the volumetric representation of 3D point clouds,each voxel is a 4D tensor,then use 3D Convolution Neural Network(CNN) to extract 3D voxel features directly on sparse point clouds, and PointPillars\cite{lang2019pointpillars} to learn the features from vertical columns(Pillars) and encodes the learned features as a pesudo image,then a 2D object detection pipeline is used to predict 3D bounding boxes from bird's eye view(BEV).In contract point-based networks directly work on raw point clouds without any voxelization or projection,the point-based methods mainly uses PointNet\cite{qi2017pointnet} or PointNet++\cite{qi2017pointnet++} to encode 3D points,F-PointNets\cite{qi2018frustum} is pioneering work in this direction, It generates a proposal for each 2D boxes in 2D image,then use PointNet to learn each cropped 3D frustum point cloud proposal feature, and others use more strategies 3DSSD\cite{yang20203dssd},PointRCNN\cite{shi2019pointrcnn},STD\cite{yang2019std} to deal with point clouds to predict 3D object information,most point-based methods were use PointNet series. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{{Multi-\changes{sensors} Fusion-based 3D Object Detection}}
\subsection{{Multi-sensors Fusion-based 3D Object Detection}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{The LiDAR can provide precision distance information while the textures information has been lost. The camera sensor is just the opposite. Multi-sensor fusion-based approaches have been proposed to utilize the advantages of both LiDAR and textures information with different types of sensors. According to \cite{nie2020multimodality}, multi-modal fusion approaches can be categorized into model-based \cite{muresan2020stabilization} and data-based methods based on the way of fusing the sensor data. Generally, model-based methods have been widely utilized for tracking \cite{muresan2019multi} while data-based approaches are more commonly applied to environment perception tasks like object detection \cite{du2018general,pang2020clocs,chen2017multi}.In general, all fusion-based approaches to object detection can be categorized into three types: early fusion \cite{du2018general}, late fusion \cite{pang2020clocs} and deep fusion \cite{chen2017multi}. The methods in F-PointNet \cite{qi2018frustum}, PointFusion \cite{xu2018pointfusion} and \cite{du2018general} generate object proposal in the 2D image fist and then fuse the image features and point cloud for 3D BBox generation.  %\cite{du2018general} presents a two-stage early fusion approach that generates the 2D proposals from images, and then fuses them with the 3D point cloud to generate 3D information.  F-PointNet \cite{qi2018frustum} leverages the 2D proposals generated by image to get cropped frustums and refine the final 3D bounding box. Moreover, PointFusion \cite{xu2018pointfusion} processes the cropped image and points independently by a CNN and PointNet network, and designs a novel fusion network.
PointPainting \cite{vora2020pointpainting} is an approach proposed to enhance the performance of 3D point cloud object detectors by fusing semantic information from 2D images into the point cloud. In order to obtain parsing results, any SOTA approach can be used. AVOD \cite{ku2018joint}, which is a typical late fusion framework, generates features that can be shared by RPN (region proposal network) and second stage refinement network. %MV3D \cite{chen2017multi} presents a multi-view representation aggregation pipeline, which could generate proposals by deep fusion of the BEV, camera view, and front view images. CLOCs \cite{pang2020clocs} combines the output candidates before NMS (Non-Maximum Suppression) from both 2D and 3D detectors, and produces more accurate detection results by leveraging their geometric and semantic consistencies.
%\xsqcomments{Nie et al. proposed a multimodality deep fusion approach called IMF-DNN\cite{nie2020multimodality} throughout several deep neural networks(DNN) for both object detection and end-to-end predict steering angle and speed. The method verify the robustness and effective by using a real-world driving dataset.  Muresan et al. \cite{muresan2020stabilization} provide a data association approach which use multiple sensors such as LIDAR, fisheye camera, trifocal camera and radar, etc. The method can noteworthy improve the accuracy and precision of positioning with semantic information.} 
Multi-task fusion\cite{he2017mask} \cite{liang2019multi} has been proven effective in various tasks, such as jointing semantic segmentation with 3D object detection tasks as demonstrated in \cite{zhou2020joint}. Furthermore, Radar and HDMaps are also employed for improving the detection accuracy. Using the frustum-based association method, CenterFusion \cite{nabati2021centerfusion} focuses on the fusion of radar and camera sensors and associates the radar detections with objects in the image and creates radar-based feature maps to supplement the image features through a middle-fusion approach. In \cite{yang2018hdnet} and \cite{fang2021mapfusion}, the HDMaps have been utilized as a valuable source of prior information for detecting moving objects in AD scenarios.

% CLOCs \cite{pang2020clocs} fusion provides a low-complexity multi-modal fusion framework that significantly improves the performance of single-modality detectors. CLOCs operates on the combined output candidates before Non-Maximum Suppression (NMS) of any 2D and any 3D detector, and is trained to leverage their geometric and semantic consistencies to produce more accurate final 3D and 2D detection results.

% uses the image to generate proposals and refines the final bounding box in cropped frustums with PointNet. 

% PointFusion \cite{xu2018pointfusion} is also a 2D proposal-driven method,  but the cropped image and points are independently processed by a CNN and a PointNet architecture, then combined by a novel fusion network.



% uses an easy but effective strategy: retrieving the class score vector for each point by projecting them into image semantic segmentation results, and feeding the concatenated attribution to 3D object detection framework. 
% F-PointNet \cite{qi2018frustum} uses the image to generate proposals and refines the final bounding box in cropped frustums with PointNet. PointFusion \cite{xu2018pointfusion} is also a 2D proposal-driven method,  but the cropped image and points are independently processed by a CNN and a PointNet architecture, then combined by a novel fusion network.
% AVOD \cite{ku2018joint}, which is a typical late fusion framework, takes LiDAR point clouds and RGB images as input, to generate features shared by RPN (region proposal network) and the refined network. MV3D \cite{chen2017multi} proposes a multi-view representation including BEV, camera view and front view image. The framework generates proposals from the BEV and deeply fuses the features from other views. CLOCs \cite{pang2020clocs} fusion provides
% a low-complexity multi-modal fusion framework that significantly improves the performance of single-modality detectors. CLOCs operates on the combined output candidates before Non-Maximum Suppression (NMS) of any 2D and any 3D
% detector, and is trained to leverage their geometric and semantic consistencies to produce more accurate final 3D and 2D detection results.

% Multi-task fusion\cite{he2017mask} \cite{liang2019multi} is also an effective technology, e.g., \cite{zhou2020joint} jointing the semantic segmentation with 3D object detection tasks to further improve the performance. 


% Furthermore, Radar and Map are also candidate for multi-modal fusion. CenterFusion \cite{nabati2021centerfusion} focus on the fusion of radar and camera sensor and associate the radar detections to objects on the image using a frustum-based association method, and creates radar-based feature maps to complement the image features in a middlefusion approach. In \cite{yang2018hdnet} and \cite{fang2021mapfusion}, the HD Maps are also taken as an strong prior information for movable object detection in autonomous driving scenario. 


% Different from the above methods, PointPainting \cite{vora2020pointpainting} uses an easy but effective strategy: retrieving the class score vector for each point by projecting them into image semantic segmentation results, and feeding the concatenated attribution to 3D object detection framework. 

%g, a novel sequential fusion method that paints lidar point clouds with image based semantics


%Many approaches have been proposed for 3D object detection to leverage fusion strategy for better performance. MV3D \cite{chen2017multi} employs a compact multi-view representation to encode the sparse 3D point cloud, which is composed of 3D object proposal generation and multi-view feature fusion. Meanwhile, using LIDAR point cloud and RGB image as input, AVOD \cite{ku2018joint} proposes neural network architecture for 3D object detection, which consists of a region proposal network (RPN) and a second stage detector network. Besides, to solve the problem of localizing objects in point clouds of large-scale scenes, Frustum pointnets \cite{qi2018frustum} leverages both mature 2D object detectors and advanced 3D deep learning for 3D object detection with RGB-D data as input. 

%F-PointNets\cite{qi2018frustum}

%proposes a simple but practical detection framework to jointly predict the 3D BBox and instance segmentation. PointPainting \cite{vora2020pointpainting}.




==> Files/03_methods.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multi-Sem Fusion Framework} \label{sec:method}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
As shown in \figref{Fig:PointPainting} provides an overview of the \textit{Multi-Sem Fusion} framework which is designed to fully leverage the information obtained from a variety of sensors, we advocate fusing them at two different levels. First, the two types of information are early fused with the \textit{PointPainting} technique by painting the point cloud with both the 2D and 3D semantic parsing results. To handle the {inaccurate segmentation} results, an AAF module is proposed to learn an attention score for different sensors {for the following fusion purpose}. By taking the points {together with fused semantic information} as inputs, deep features can be extracted from the backbone network. By considering that different size object requires different levels features, a novel DFF module is proposed to enrich features from the backbone with different levels for exploring the global context information and the local spatial details in a deep way. As illustrated in \figref{Fig:PointPainting}, Our framework comprises three primary models: a multi-modal semantic segmentation module, an Adaptive-attention fusion (AAF) module, and a deep feature fusion (DFF) module. To obtain the semantic segmentation from both RGB images and LiDAR point clouds, we can leverage any existing 2D and 3D scene parsing approaches. Then the 2D and 3D semantic information are fused by the AAF module. Bypassing the points {together with fused semantic labels} into the backbone network, the DFF module is used to {further improve the results by aggregating the features information within various receptive fields and a channel attention module.}
    
%We describe the architecture of our \textit{FusionPainting} framework in \figref{Fig:PointPainting}. We propose to leverage both the 2D images and 3D point clouds information for obtaining accurate 3D locations of obstacles in the autonomous driving scenarios. Here, the fusion process is achieved by adaptively integrating 2D and 3D information at the semantic level. As shown in \figref{Fig:PointPainting}, the proposed framework consists of three models as a multi-modal semantic segmentation module, an adaptive attention module, and a 3D detector module. First, any off-the-shelf 2D and 3D segmentors can be employed to obtain the semantic segmentation from the RGB image and LiDAR point clouds respectively. Then a simple but effective attention strategy is proposed to sufficiently benefit the merits and suppress the drawbacks of the 2D and 3D semantic results. Finally, painted 3D point clouds with enhanced semantic labels are sent to modern 3D object detectors for achieving the final detection results.    



\begin{figure*}[ht]
    \centering
	\includegraphics[width=1\textwidth]{Figs/Attention.pdf}
	\caption{The architecture of the proposed AAF module for 2D/3D semantic fusion. The proposed framework leverages the input points and 2D/3D semantic results to learn attention scores throughout an adaptive attention network, which are then used to paint the raw points or voxel with adaptive 2D/3D semantic labels}
	\label{Fig:attention_module}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{2D/3D Semantic Parsing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\textit{{2D Image Parsing.}} By incorporating 2D images into our approach, we can leverage their rich texture and color information to complement the analysis of 3D point clouds. For acquiring 2D semantic labels, a modern semantic segmentation method is employed here for generating pixel-wise segmentation results. More importantly, the proposed framework is allowing for the use of a wide range of state-of-the-art segmentation approaches without requiring modification. This agnostic approach enables researchers and practitioners to more easily leverage their preferred segmentation models and techniques (e.g., \cite{choudhury2018segmentation,zhao2017pyramid,chen2019hybrid,shelhamer2017fully,Howard_2019_ICCV}, etc). {We employ Deeplabv3+ \cite{choudhury2018segmentation} for generating the semantic results here.} The network takes 2D images as input and produces pixel-wise semantic classes scores for both the foreground and background categories. {Assuming that the obtained semantic map is $S \in \mathbb{R}^{w\times h \times m}$, where $(w, h)$ is the input image size and $m$ is the number of category. By employing the intrinsic and extrinsic matrices, the 2D semantic information can be easily re-projected into the 3D point cloud. Specifically, by assuming that} the parameter of the intrinsic matrix is $\mathbf{K} \in \mathbb{R}^{3\times 3}$, extrinsic matrix $\mathbf{M}\in \mathbb{R}^{3\times 4}$ and the original 3D points clouds is $\mathbf{P}\in \mathbb{R}^{N\times 3}$, we can derive the projection of the LiDAR 3D point cloud onto the camera as Eq.\eqref{eq.projection} shown:
\begin{equation} \label{eq.projection}
	 {\mathbf{P}}^{'} = \text{Proj}(\mathbf{K}, \mathbf{M}, \mathbf{P}),
\end{equation} 
where $\mathbf{P}^{'}$ represent the LIDAR point in camera coordinates and ``Proj'' denote the projection process. {By this projection, we can assign the semantic segmentation results obtained from the 2D image to their corresponding 3D points which is denoted by $\mathbf{P}_{2D}\in \mathbb{R}^{N\times m}$.


%Finally, we got the 2D segmentation map  $S \in \mathbb{R}^{w\times h \times m}$ from 2D image segmentor, where $w, h$ denote width and length of the input image respectively, $m$ is the number of semantic classes. 


%In order to each point category in point clouds. We are following the procedures in the work of ~\cite{vora2020pointpainting}~\cite{vora2020pointpainting}, the 3D point clouds are projected onto the corresponding pixel-wise 2D segmentation mask with the intrinsic and extrinsic projection matrices. We take intrinsic matrix as $\mathbf{K} \in \mathbb{R}^{3\times 3}$, the extrinsic matrix is $\mathbf{M}\in \mathbb{R}^{3\times 4}$ and the original 3D points clouds is $\mathbf{P}\in \mathbb{R}^{N\times 3}$, the projection of 3D point clouds from LiDAR coordinate to camera coordinate can be obtained as follow Eq. (\ref{eq.projection}).
%\begin{equation} \label{eq.projection}
%	 {\mathbf{P}}^{'} = \text{Proj}(\mathbf{K}, \mathbf{M}, \mathbf{P}),
%\end{equation} 
%where $\mathbf{P}^{'}$ denote that final projected point in camera coordinate and the ``Proj'' is the whole 2D/3D projection process. With this projection, the semantic results in the 2D image can be assigned to its corresponding 3D point cloud.

\textit{{3D Point Cloud Parsing.}} As we have mentioned above, {parsing results from the point clouds can well overcome the boundary blur influence while keeping the distance information. Similar to the 2D image segmentation, any SOTA 3D parsing approach can be employed here \cite{zhang2020polarnet,cheng20212,xu2021rpvnet}. We employ the Cylinder3D \cite{cong2021input} for generating the semantic results because of its impressive performance on the AD scenario.}
%Specifically, Cylinder3D transforms the point cloud into the cylindrical coordinates first and then an asymmetrical 3D convolution module is employed to extract features for the segmentation task.  
{More importantly, the ground truth point-wise semantic annotations can be generated from the 3D object bounding boxes roughly as \cite{shi2019pointrcnn} while any extra semantic annotations are not necessary.} Specifically, for assigning semantic labels to the 3D points, we directly assign class labels to the points inside a 3D bounding box for foreground instances, while considering points outside all the 3D bounding boxes as the background. This approach enables our proposed framework to work directly on 3D detection benchmarks without requiring additional point-wise semantic annotations. After training the network, we will obtain the parsing results which is denoted by $\mathbf{P}_{3D}\in \mathbb{R}^{N\times m}$. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Adaptive Attention-based 2D/3D Semantic Fusion} \label{subsec:shallow_fusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{As mentioned in previous work PointPainting, 2D semantic segmentation network have achieved impressive performance,} however, the {blurring effect at the shape boundary} is also serious due to the restricted resolution of the feature map (e.g., $\frac{1}{4}$ of the original image size). Therefore, {the point clouds with 2D semantic segmentation} usually has misclassified regions around the objects' boundary. For example, the frustum region is illustrated in the sub-fig.~\ref{Fig:2DSeg_in_3d} (a) behind the big truck {has been totally misclassified}. On the contrary, the {parsing results} from the 3D point clouds usually perform a clear and accurate object boundary without blurring effect e.g., sub-fig.~\ref{Fig:2DSeg_in_3d}(b). However, the disadvantages of the 3D segmentor are also obvious. One drawback is that without the color and texture information, the 3D segmentor is difficult to distinguish these categories with similar shapes from the point cloud-only. In order to boost advantages while suppressing disadvantages, an AAF module has been proposed to adaptively combine the 2D/3D semantic segmentation results. Then the Optimized semantic information is ready for the following 3D object detectors backbone to further extract the enhanced feature to improve the final object detection accuracy results.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{figure*}[h]
	\centering
  	\includegraphics[width=0.95\textwidth]{Figs/DFF.pdf}
	\centering
	\caption{An illustration of the proposed Deep Feature Fusion (DFF) module which includes one \textit{fusion} module and one \textit{channel attention} module respectively. The \textit{fusion} module includes two branches for producing features with different field-of-view.}
	\label{fig:deep_feature_fusion}
\end{figure*}

\textbf{AAF Module.} The detailed architecture of the proposed AAF module is depicted in Fig.~\ref{Fig:attention_module}. The input point clouds is defining as a set of points $\{\mathbf{P}_i, i=1,2,3...N\}$, with each point $\mathbf{P}_i$ containing $(x, y, z)$ coordinates and other optional information such as intensity. In the following context, we'll focus solely on the coordinates that meaning only the coordinates $(x, y, z)$ are considered as input data. Our objective is to develop an efficient strategy for integrating semantic information from both 2D images and 3D point clouds.}. Here, we propose a novel approach that employ adaptive attention fusion(AAF) module to learn each cell attention score in voxel level or point level to adaptively combine the two types of semantic results. Specifically, the module 
begins by concatenating the point clouds coordinate attributes $(x, y, z)$ and 2D/3D semantic segmentation labels to obtain a fused point clouds with the shape of $N\times (2m+3)$. In order to reduce memory consumption during the fusion process, we have implemented a voxel-level fusion approach instead of operating at the point level. To achieve this, the point clouds are first evenly divided into voxels, and the voxels are represented as $\{ V_i, i=1,2,3...E\}$, where $E$ is the overall count of the voxels. Specially, each voxel cell $V_{i}  = (\textbf{P}_i, \textbf{V}^{i}_{2D}, \textbf{V}^{i}_{3D}) \in \mathbb{R} ^{M \times(2m+3)}$ containing a fixed number of $M$ points, and each point attributes consist of $\textbf{P}_i$, $\textbf{V}^{i}_{2D}$, $\textbf{V}^{i}_{3D}$ which represent point coordinates, predicted 2D and 3D semantic segmentation results vector respectively. To ensure consistency across voxels, we utilize a sampling technique to maintain a fixed number of points in each voxel.
%\xsqcomments{And here we also project $\mathbf{P}_{3D}$, $\mathbf{P}_{2D}$ into voxel level \{$\mathbf{V}_{3D}, \mathbf{V}_{2D}\} \in \mathbb{R}^{E\times M\times m}$}. 
Subsequently, we utilize local and global feature aggregation techniques to calculate attention weights for each voxel, which help to determine the relative importance of 2D and 3D semantic segmentation labels. In other words, the AFF module chooses which category of 2D/3D semantic information should be trusted in the voxel.

In order to get local features, we utilize a PointNet~\cite{qi2017pointnet}-like module to extract voxel-wise information within each non-empty voxel. Specifically, for the $i$-th voxel, the corresponding local feature is represented as: 
\begin{equation} \label{local_feature}
 V_i = f(p_1, p_2,  \cdots , p_M) =
 \max_{i=1,...,M} \{\text{MLP}_{l}(p_{i^{'}})\} \in \mathbb{R}^{C_1},
\end{equation}
{where $\{p_{i^{'}}, i^{'}=1,2,3...M\}$ indicates the LIDAR points insize each voxel}. $\text{MLP}_{l}(\cdot)$ and ${max}$ represent the muti-layer perception (MLP) and max-pooling module, respectively. Specifically, $\text{MLP}_{l}(\cdot)$ is composed of a linear layer, a batch normalization layer, an activation layer. Throughout the network, we got outputs for each voxel local feature with $C_1$ channels. For global feature information, we aggregate information based on the $E$ voxels where $E$ is the total number of voxels. First, we employ a $\text{MLP}_{g}(\cdot)$ module to rich each voxel features from $C_1$ dimensions to $C_2$. Then, we apply another PointNet-like module on all the voxels as follows expression:
\begin{equation} \label{global_feature}
V_{global} = f(V_1, V_2, \cdots ,V_E) = \max_{i=1,...,E} \{\text{MLP}_{g}(V_i)\} \in \mathbb{R}^{C_2}.
\end{equation}
To obtain the final fused local and global features, we expand the global feature vector $V_{global}$ to the same size as the number of voxels and then concatenate it with each local feature $V_i$. This operation creates a combined feature representation for each voxel that captures both local and global information as $V_{gl}\in \mathbb{R}^{E \times{(C_1 + C_2)}}$.
 

{After getting} fused features $V_{gl}$ from the network, we can estimate an attention score of two kinds of semantic information results for each point in voxel throughout another MLP module $\text{MLP}_{att}(\cdot)$ on $V_{gl}$ and a Sigmod activation function $\sigma(\cdot)$. Then, we multiply the resulting attention confidence score with corresponding one-hot semantic vectors for each voxel, as shown in Eq. (\ref{attention_2d}), Eq. (\ref{attention_3d}):
\begin{equation} \label{attention_2d}
	    \mathbf{V}^{i}_{a.S}  = \mathbf{V}^{i}_{2D} \times \sigma{(\text{MLP}_{att}(V^{i}_{gl})}) ,
\end{equation} 
\begin{equation}\label{attention_3d}
	    \mathbf{V}^{i}_{a.T} = \mathbf{V}^{i}_{3D} \times (1-\sigma{(\text{MLP}_{att}(V^{i}_{gl}})))
\end{equation} 
where $\mathbf{V}^{i}_{2D}$ and $\mathbf{V}^{i}_{3D}$ are the point labels in each voxel from 2D and 3D semantic segmentation results which are encoded with {one-hot} format. {The final semantic vector $V^{i}_{final}$ of each voxel can be obtained by concatenating or element-wise addition of $\mathbf{V}^{i}_{a.T}$ and $\mathbf{V}^{i}_{a.S}$.} 


%\xsqcomments{After Sigmoid operation the value will at the range from 0 to 1, the weighted semantic information $\mathbf{V}_{a.S}$ and $\mathbf{V}_{a.T}$ taking by multiplying with it corresponding semantic result vector.}
%\begin{equation}\label{attention_final}
%	    \mathbf{V}_{final} = \mathbf{V}_{a.T} + \mathbf{V}_{a.S}
%\end{equation}

%\xsqcomments{The enhanced fusion information will be added together as Eq. \eqref{attention_final} shown. And then fuse it with raw voxel features like $(x, y, z)$. Finally, we got $ \mathbf{V}_{final} \in \mathbb{R}^{E \times M \times (m+3)}$ which contains the adaptively weighted information from both 2D and 3D semantic labels.}

\iffalse
\xsqcomments{
 Taking KITTI dataset as example, for a certain point, supposed that we got 2D/3D semantic segmentation after encoder to {one-hot} vector are as follows:
\begin{equation}\label{p_2d_onehot}
	    \mathbf{P}_{2D} = [0,0,1,0]
\end{equation} 
\begin{equation}\label{p_3d_onehot}
	    \mathbf{P}_{3D} = [0,0,0,1]
\end{equation} 
}
\xsqcomments{In the equation, different dimensions denote the category of 'Car', 'Pedestrian', 'Cyclist' and 'Background', respectively. Here, each point both have 2D/3D semantic information, and '1' present which category this point belong to. If the weight of score to trust 2D/3D semantic information is 0.2 and 0.8 for this certain point, after Eq.(\ref{attention_2d}), Eq(\ref{attention_3d}), we got follow present:
\begin{equation} \label{attention_2d_final}
	    \mathbf{P}_{a.S}  = [0,0,1,0] \otimes 0.2 = [0,0,0.2,0],
\end{equation} 
\begin{equation}\label{attention_3d_final}
	    \mathbf{P}_{a.T} =[0,0,0,1] \otimes 0.8 = [0,0,0,0.8]
\end{equation} 
}
\xsqcomments{Different with previous conference, we plus them together as described in Eq.(\ref{attention_final}).
\begin{equation}\label{attention_final}
	    \mathbf{P}_{final} = \mathbf{P}_{a.T} + \mathbf{P}_{a.S} = [0,0.2,0,0.8]
\end{equation}
We can find the weight of 'background' from 3D semantic information in more than 'Pedestrian' which from 3D semantic. The results denote that 3D semantic information can greatly correct the mistakes from 2D boundary-blurring effect happened in 2D semantic segmentation. On the contrary, 2D semantic information will correct the miss-classified which happened in 3D semantic segmentation if the score of 2D is more than 3D semantic segmentation. Then we fused $\mathbf{P}_{fianl} \in \mathbb{R}^{N \times M \times m}$ with raw point $P$ in each voxel to replace the voxels shape $\widehat{V}_m\in \mathbb{R}^{N\times M \times (3 + 2m)}$, where $m, M$ denote semantic classes number and points number in voxel. Finally, $\hat{V_m}$ contains the adaptively fused information from 2D and 3D semantic labels.}
\fi




\begin{table*}[ht]
\centering
\renewcommand\arraystretch{1.1}
\resizebox{0.85\textwidth}{!}
{
\begin{tabular}{r|c|lll|lll|lll}
\hline
\multicolumn{1}{r|}{\multirow{2}{*}{$\textbf{Methods}$}} &\multicolumn{1}{c|}{\multirow{2}{*}{$\textbf{mAP}$ (Mod.)(\%)}} &
\multicolumn{3}{c|}{$\textbf{Car}$ $AP_{70}(\%)$} & 
\multicolumn{3}{c|}{$\textbf{Pedestrian}$ $AP_{70}(\%)$} & 
\multicolumn{3}{c}{$\textbf{Cyclist}$ $AP_{70}(\%)$}  \\ %\cline{2-14} 

{} & {} & {Easy} & {Mod.} & {Hard} & %{l}{} & 
{Easy} & {Mod.} & {Hard} & %{l|}{} & 
{Easy} & {Mod.} & {Hard}  \\ \hline  \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{SECOND } & {66.64} & 
%{} & 
{90.04} & {81.22} & {78.22} & %{} & 
{56.34} & {52.40} & {46.52} & %{} & 
83.94 & 66.31 & {62.37} \\
%%%%%%%%%%%%%%%%%%%%%
{SECOND $^{\ast}$} & {68.11} & 
%SECOND  & {68.11} & 
%{} & 
{91.04} & {82.31} & {79.31} & %{} &
 {59.28} & {54.18} & {50.20} & %{} & 
85.11 & 67.52 & {63.36} \\ %\cdashline{2-14}[2pt/2pt]
%%%%%%%%%%%%%%%%%%%
{Improvement} & \R{+1.47} & 
%{} & 
\R{+1.00} & \R{+1.09} & \R{+1.09} & %{} & 
\R{+2.94} & \R{+1.78} & \R{+3.68} & %{} & 
\R{+1.17} & \R{+1.54} & \R{+0.99} \\ \hline 

{Pointpillars} & {62.90} 
%& {} 
& {87.59} & {78.17} & {75.23} & %{} &
 {53.58} & {47.58} & {44.04} & %{} & 
{82.21} & {62.95} & {58.66} \\
%{PointPillars} & {65.78} & 
{PointPillars$^{\star}$} & {65.78} &%{} &
{89.58} & {78.60} & {75.63} & %{} & 
{60.22} & {54.23} & {49.49} & %{} & 
84.83 & 64.50 & {60.17} \\ %\cdashline{2-14}[2pt/2pt]

{Improvement} & \R{+2.88} & 
%{} & 
\R{+1.99} & \R{+0.43} & \R{+0.4} & %{} & 
\R{+6.64} & \R{+6.65} & \R{+5.45} & %{} & 
\R{+2.62} & \R{+1.55} & \R{+1.51} \\ \hline

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{PV-RCNN} & {71.82} &
%{} & 
{92.23} & {83.10} & {82.42} & %{} & 
{65.68} & {59.29} & {53.99} & %{} & 
91.57 & 73.06 & {69.80} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{PV-RCNN$^{\ast}$} & {73.95} & 
%{PV-RCNN} & {73.95} & 
%{} & 
{91.85} & {84.59} & {82.66} & 
{69.12} & {61.61} & {55.96} & 
94.90 & 75.65 & {71.03} \\ 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{Improvement} & \R{+2.13} & 
\G{-0.38} & \R{+1.49} & \R{+0.24} & %{} & 
\R{+3.44} & \R{+2.32} & \R{+1.97} & %{} & 
\R{+3.33} & \R{+2.59} & \R{+1.23} \\ \hline
\end{tabular}
}
\caption{3D object detection evaluation on KITTI ``val'' split on different baseline approaches, where $^{\star}$ represents the boosted baseline by adding the proposed fusion modules. ``Easy'', ``Mod.'' and ``Hard'' represent the three difficult levels defined by official benchmark and $\textbf{mAP}$ (Mod.) represents the average $\textbf{AP}$ of ``Car'', ``Pedestrian'' and ``Cyclist'' on ``Mod.'' level. For easy understanding, we also highlight the improvements with different colors, where red represents an increase and green represents a decrease compared to the baseline method. This table is better to be viewed in color mode.}
\label{tab:kitti_3D_detection}
\end{table*}

\begin{table*}[!ht]
\centering
\renewcommand\arraystretch{1.1}
\resizebox{0.85\textwidth}{!}
{
    \begin{tabular}{r|c| ccc | ccc| ccc}
    \hline
    \multirow{2}{*}{$\textbf{Methods}$} &\multirow{2}{*}{$\textbf{mAP}$ (Mod.)(\%)} &
    \multicolumn{3}{c|}{$\textbf{Car}$ $AP_{70}(\%)$} &
    \multicolumn{3}{c|}{$\textbf{Pedestrian}$ $AP_{70}(\%)$} & 
    \multicolumn{3}{c}{$\textbf{Cyclist}$ $AP_{70}(\%)$}  \\ %\cline{2-14} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    {} & {} & {Easy} & {Mod.} & {Hard} & 
    {Easy} & {Mod.} & {Hard} & 
    {Easy} & {Mod.} & {Hard}  \\ \hline  \hline 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    {SECOND}  & {71.95}  
    & {92.31} & {88.99} & {86.59}  
    & {60.5} & {56.21} & {51.25}  
    & {87.30} & {70.65} & {66.63} \\
    SECOND $^{\star}$ & {73.72}  
    & {94.70} & {91.62} & {88.35}  
    & {63.95} & {59.66} & {55.81}  
    & {91.95} & {73.28} & {67.75} \\
    {Improvement} & \RED{{+2..90}} 
    & \RED{+2.39} & \RED{+2.63}  & \RED{+1.76}  
    & \RED{+3.45} & \RED{+3.45} & \RED{+4.56} 
    & \RED{+4.65} & \RED{+2.63} & \RED{+1.12} \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    {Pointpillars } & {69.18}  
    & {92.50} & {87.80} & {87.55}  
    & {58.58} & {52.88} & {48.30} 
    & {86.77} & {66.87} & {62.46} \\
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    PointPillars $^{\star}$  & {72.13}  
    & {94.39} & {87.65} & {89.86}  
    & {64.84} & {59.57} & {55.16}  
    & {89.55} & {69.18} & {64.65} \\
    {Improvement} & \RED{{+2.95}}  
    & \RED{+1.89} & \GRE{-0.15} & \RED{+2.31}  
    & \RED{+6.26} & \RED{+6.69} & \RED{+6.86}  
    & \RED{+2.78} & \RED{+2.31} & \RED{+2.19} \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    {PV-RCNN}  & {76.23}  
    & {94.50} & {90.62} & {88.53}  
    & {68.67} & {62.49} & {58.01} 
    & {92.76} & {75.59} & {71.06} \\
    PV-RCNN $^{\star}$ & {78.17}  
    & {94.86} & {90.87} & {88.88}  
    & {71.99} & {64.71} & {59.01} 
    & {96.35} & {78.93} & {74.51} \\
    {Improvement} & \RED{{+1.94}}  
    & \RED{+0.36} & \RED{+0.25} & \RED{+0.35}
    & \RED{+3.32} & \RED{+2.22} & \RED{+1.00} 
    & \RED{+3.59} & \RED{+3.34} & \RED{+3.45} \\ \hline
    \end{tabular}
}
\caption{Evaluation of bird's-eye view object detection on KITTI ``val'' split with different baselines. Similar to the 3D detection, the red color represents an increase and the green color represents a decrease compared to the baseline method. This table is also better to be viewed in color mode.}
\label{tab:KITTI_BEV_detection}
\end{table*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Deep Feature Fusion Module} \label{subsec:deep_fusion}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In AD scenarios, determining the identity and location of objects is crucial for the subsequent planning and control modules. Therefore, it is not only necessary to recognize what objects are present, but also where they are located. In typical object detection frameworks, they correspond to the classification and regression branches respectively. Empirically, global context information is important to recognize the specific class attributes. On the contrary, the object's attributes (e.g., dimension, orientation, and precise location, etc) regression branch prioritize the capture of detailed spatial information around the ROI (region of interest) in a relatively small range. For accurate kinds of size object detection, therefore various scales receptive fields are necessary. This issue has been considered in most object detection frameworks. However, how to use various fields of view fields in an efficient way is vitally important.

To handle this kind of issue, a specific DFF module is proposed to aggregate both the low-level and high-level features with different receptive fields. 
The \figref{fig:deep_feature_fusion} shows the architecture of the DFF module. First, the backbone features $\textbf{F}^{0}_B$ from the feature extractor pass the \textit{Conv\_block1} with several convolution layers to obtain the $\textbf{F}^{1}_B$ as a basic feature. %Here, ``Conv\_block1'' as an example to explain the details of sub-Network, 
Here, \textit{Conv\_block1} has four Conv modules and the first $conv$ module takes $C$ channels as input and outputs 128 channels, and the following three $convs$ share the same input {channels} and output channels. For each $conv$ module in the \figref{fig:deep_feature_fusion}, it consists one $Con2d$, a batch normalization layer, and a Rectified Linear Unit (ReLU) activation layer. For easy understanding, we have given the stride and kernel size for each $conv$ operation at the bottom of \figref{fig:deep_feature_fusion}. Then, the feature $\textbf{F}^{1}_B$ will pass two branches to obtain the features with different receptive fields. For one branch, the features are down-sampled into $1/2$ size with $Conv-block2$ first and then pass the $Conv2$ operation. Finally, the outputs are up-sampled into the feature map $F_{R}^{L}\in \mathbb{R}^{H \times W \times C' }$ with $Deconv2$. For the other branch, $F^{1}_{B}$ will pass $Covn3$ and $Conv4$ to obtain the features of $F_{R}^{S}$ consecutively. And the shape of the output $F_{R}^{L}$ is the same as $F_{R}^{S}$. Specially, $C'$ can be C.

After adding the high-level and low-level features element-wisely, a channel-attention (CA) module like \cite{fu2019dual} is employed to further fuse both of them. The architecture of the module can be found in \figref{fig:deep_feature_fusion} which is named 'CA'. Usually, the channel feature from low-level to high-level throughout the backbone will take the loss of information. In order to minimize this influence, we utilize the CA module here to selectively emphasize interdependent channel maps by integrating relative features among all channel maps. Specially, the enhanced feature  $F_{E}^{F}$ which is reshaped to $\mathbb{R}^{C \times{N}}$, where $N=H\times W$ is the pixel numbers of each channel. can be as the original feature sent into the module. Then, the reshaped feature, which is denoted as:  the $\textbf{F}^{F}_E$ can be fused better in a deep way. Finally, $\textbf{F}^{G}_E$ is taken as the inputs for the following classification and regression heads. 


%and also pass triple same independent parameters conv module from 128 channels and output same. Especially each Conv module in the Figure.\ref{fig:deep_feature_fusion} consists of a Con2d, a batch normalization layer, and a Rectified Linear Unit (ReLU) activation layer.

%We can see more details in the figure, such as stride and kernel size. etc. Then, the feature $\textbf{F}^{1}_B$ will pass parallels two branches to obtain the different receptive field features $\textbf{F}^{S}_R$ and decoded to original size feature map $\textbf{F}^{L}_R$ respectively. After adding them element-wisely, a special similar with channel-attention module described in Dual-attention \cite{fu2019dual} is employed to fuse the two kinds of features for obtaining the enhanced features $\textbf{F}^{G}_E$. The channel attention module selectively emphasizes interdependent channel maps by integrating relative features among all channel maps, so the fused receptive field feature $\textbf{F}^{F}_E$ can be fused better in a deep way. Finally, the enhanced features are taken as the inputs for the following classification and regression heads.}  
 

%In the experiments section, we will show that our proposed framework achieve significant performance improvement over state-of-the-art 3D detectors.
% We take raw point cloud with corresponding both of 2d and 3d semantic information as input data,then through adaptive module framework as show in Fig.\ref{Fig:attention_module},dynamic learn the confidence of each voxel for better performance of detection.

% Adaptive fusion work is an early fusion approach, in which fusion of two significant complementary source information 2D and 3D segmentation result of each point in point cloud.We take raw point cloud with corresponding both of 2d and 3d semantic information as input data,then through adaptive module framework as show in Fig.\ref{Fig:attention_module},dynamic learn the confidence of each voxel for better performance of detection.Adaptive fusion work derived from \textit{Channel Feature Aggregation} and \textit{Local and Global voxel information Aggregation},the details as follow.

% We take point cloud into voxel presentation.Suppose that the point cloud encompasses 3D space with range D, H and W along the Z, Y, and X axis respectively each grid size $V_D,V_H,V_W$.Finally we get 3D grid dimension $D'=D/V_D,H'=H/V_H,W'=W/V_W$.take n,K as maximum number of voxel and point of non-empty voxel respectively, where \{$N \le n,N,n,K \in \mathbb{R}$\}, specially we define K as invariant constant,if number of point in each voxel over K,we will randomly sampled point number to K,Conversely,if sample has too little  data than K,zero padding is applied,finally we got point cloud to $\text{V} = \{ V_{1},V_{2}, .... ,V_{M}\}$, where $V_{m} \in \mathbb{R} ^{N \times C}$ present m-th voxel of V.

%Multi-modal Segmentation Fusion Network (MSFN)

% As showed in Fig.~\ref{Fig:2DSeg_in_3d},image B is differ between projected 2d and 3d semantic LIDAR point,where green denote that point label from 2d and 3d are same ,and red is differ,we can easily see that most of differ point label is the frustum effect from 2d,and same points classed wrong from 3D segmentation, Compare with 3D semantic segmentation 2d result has serious and obvious tail or frustum effect,but has high recall for foreground segmentation.Our Adaptive-MutiSegFusionNet is aim to fusion the advantage both of 2d and 3d segmentation.


% \textbf{Channel Feature Aggregation:} The voxel set $V \in \mathbb{R^{N \times K \times C}}$ as we definite above,where N,K,C present number of voxel,point in each voxel and point feature which combine 2D and 3D semantic segmentation respectively.It is necessary for a multi-sensor system to include a mechanism encouraging on the different source data to compensate for each other.Here $1 \times 1$ convolutional layers are used to increase the dimension of point feature,scripts 1 and C of $W_1$,$E^{C}$ denote that we use $1 \times 1$ convolution on C-channel,i.e.:$$ E^{C1} = R(B(W_1E^C) $$ where $E^{C_{1}}$ is the result from $C$-channel to $C_{1}$-channel after convolutional network,B is the batch nomalization(BN),R is a rectified linear unit(ReLU) activation function.there we get a set of encoding feature shape as $[N,K,C_1$].

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{3D Object Detection Framework} \label{subsec:3d_detector}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{The proposed AAF and DFF modules are }detector independent and any off-the-shelf 3D object detectors can be directly employed as the baseline of our proposed framework. The 3D detector receives the points or voxels produced by the AAF module as inputs and can keep backbone structures unchanged to {obtain the backbone features. Then, the backbone features are boosted by passing the proposed DFF module. Finally, detection results are generated from the classification and regression heads.}










==> Files/04_experiments.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Results} \label{sec:experiments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To verify the effectiveness of our proposed framework, we evaluate it on two large-scale 3D object detection dataset in AD scenarios as KITTI \cite{geiger2012we} and nuScenes \cite{caesar2020nuscenes}. Furthermore, {the proposed modules is also evaluated on different kinds of baselines} for verifying its generalizability, including SECOND \cite{yan2018second}, PointPilars \cite{lang2019pointpillars} and PVRCNN \cite{shi2020pv}, etc.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation on KITTI Dataset} \label{subsec:eval_kitti}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
\textit{KITTI} is one of the most popular benchmarks for 3D object detection in AD, which contains 7481 samples for training and 7518 samples for testing. The objects in each class are divided into three difficulty levels as ``easy'', ``moderate'', and ``hard'', according to the object size, the occlusion ratio, and the truncation level. Since the ground truth annotations of the test samples are not available and the access to the test server is limited, we follow the idea in~\cite{chen2017multi} and split the training data into ``train'' and ``val'' where each set contains 3712 and 3769 samples respectively. In this dataset, both the LiDAR point clouds and the RGB images have been provided. In addition, both the intrinsic parameters and extrinsic parameters between different sensors have been given. %For the object detection task, multiple stereo frames have been provided while only a single image from the left camera at the current frame is used in our approach.



\begin{table*}[ht!]
%\renewcommand\arraystretch{1.3}
\centering
\normalsize
%\renewcommand\arraystretch{1.1}
\resizebox{1\textwidth}{!}
{
	\begin{tabular}{l | c | c | c c c c c c c c c c}
	\hline
    {\multirow{2}{*}{Methods}} &
    {\multirow{2}{*}{\textbf{NDS} (\%)}} &
    {\multirow{2}{*}{\textbf{mAP} (\%)}} & 
    \multicolumn{10}{c}{\textbf{AP} (\%)} \\
    {} &  {} & {} & {Car} & {Pedestrian} &{Bus} &{Barrier} & {T.C.} &
    {Truck} & {Trailer} & {Moto.} & {Cons.} &
    {Bicycle} \\ \hline \hline
    %\multicolumn{1}{l}{mAP} & \multicolumn{1}{l}{Car} & \multicolumn{1}{l}{Pedestrian} & \\
    %\textbf{Methods} & NDS & mAP & Car & Pedestrian & Bus & Barrier & T.C. & Truck & Trailer & Moto. & Cons. & Bicycle &  \hline
	SECOND \cite{yan2018second}  &61.96 &50.85 &81.61  &77.37 & 68.53 &57.75  &56.86  &51.93 &38.19 & 40.14 &17.95 & 18.16 \\
	SECOND$^{\ast}$ & 67.61  & 62.61  & 84.77  & 83.36 &72.41 &63.67 &74.99 &60.32 &42.89 &66.50 &23.59  &54.62  \\
	Improvement $\uparrow$ & \textcolor{red}{\textbf{+5.65}} & \textcolor{red}{\textbf{+11.76}} & \textcolor{red}{+3.16} & \textcolor{red}{+5.99} & \textcolor{red}{+3.88} & \textcolor{red}{+5.92} & \textcolor{red}{+18.13} & \textcolor{red}{+8.39} & \textcolor{red}{+4.70} & \textcolor{red}{+26.36} & \textcolor{red}{+5.64}& \textcolor{red}{+36.46} \\
    \hline
	PointPillars \cite{lang2019pointpillars}  & 57.50 &43.46 &80.67 &70.80 &62.01 &49.23 &44.00 &49.35 &34.86 &26.74 &11.64 &5.27 \\
	PointPillars$^{\ast}$ &66.43 & 61.75 &84.79 &83.41 &70.52 &59.42 &75.43 &57.50 &42.32 &66.97 &22.43 &54.68   \\
	Improvement $\uparrow$ & \textcolor{red} {\textbf{+8.93}} & \textcolor{red}{\textbf{+18.29}} & 
	\textcolor{red}{+4.12} & \textcolor{red}{+12.61} & \textcolor{red}{+8.51 } & \textcolor{red}{ +10.19} & \textcolor{red}{+31.43} & \textcolor{red}{+8.15} & \textcolor{red}{+7.46} & \textcolor{red}{+40.23}  & \textcolor{red}{+10.79} & \textcolor{red}{+49.41} \\
    \hline
	CenterPoint \cite{yin2021center} & 64.82 &56.53 &84.73 &83.42 &66.95 &64.56 &64.76 &54.52 &36.13 &56.81 &15.81 &37.57\\
	CenterPoint$^{\ast}$ &69.91 &65.85  &87.00 &87.95 & 71.53 &67.14 &79.89 &61.91 & 41.22 & 73.85 &23.97 &64.06\\
	Improvement $\uparrow$ & \textcolor{red}{\textbf{+5.09}} & \textcolor{red}{\textbf{+6.81}} & \textcolor{red}{+2.77} & \textcolor{red}{+4.53} & \textcolor{red}{+4.58} & \textcolor{red}{+2.58} & \textcolor{red}{+15.13} & \textcolor{red}{+7.39} & \textcolor{red}{+5.09} & \textcolor{red}{+17.04} &  \textcolor{red}{+8.16}&\textcolor{red}{+26.49} \\
    \hline
	\end{tabular}
}
\caption{\normalfont Evaluation results on nuScenes validation dataset. ``NDS'' and ``mAP'' mean nuScenes detection score and mean Average Precision. ``T.C.'', ``Moto.'' and ``Cons.'' are short for ``traffic cone'', ``motorcycle'', and ``construction vehicle'' respectively. `` * '' denotes the improved baseline by adding the proposed fusion module. The red color represents an increase compared to the baseline. This table is also better to be viewed in color mode.}
\label{tab:eval_on_nuscenes_val}
%\xsqcomments {TODO: update numbers.} 
\end{table*}




\noindent\textbf{Evaluation Metrics.} {We follow the official metrics provided by the KITTI for evaluation. ${AP}_{70}$ is used for ``Car'' category while ${AP}_{50}$ is used for ``Pedestrain'' and ``Cyclist''. }
%for the ``Car'' class, we use the metric $\textbf{AP}_\text{Car}$\textbf{70} for all the detection results which mean that only the samples in which the overlay of bounding box with ground truth is more than 70\% are considered as true positive detection. While the threshold for ``Pedestrian'' class is 0.5 (e.g., $\textbf{AP}_\text{Ped}$\textbf{50}) due to their smaller size.
Specifically, before the publication of \cite{simonelli2019disentangling}, the KITTI official benchmark used the 11 recall positions for comparison. After that, the official benchmark changes the evaluation criterion from 11-points to 40-points because the latter one is proved to be more stable than the former \cite{simonelli2019disentangling}. Therefore, we use the 40-points criterion for all the experiments here. In addition, similar to \cite{vora2020pointpainting}, the average AP (mAP) of three Classes for ``Moderate'' is also taken as an indicator for evaluating the average performance on all three classes. 

\noindent\textbf{Baselines.} Three different baselines have been used for evaluation on KITTI: 
\begin{enumerate}
    \item \textit{SECOND \cite{yan2018second}} is the first to employ the sparse convolution on the voxel-based 3D object detection framework to accelerate the efficiency of LiDAR-based 3D object detection.  
    %task and the detection efficiency has been highly improved compared to previous work such as VoxelNet \cite{zhou2018voxelnet}. 
    \item \textit{PointPillars \cite{lang2019pointpillars}} {is proposed to further improve the detection efficiency by dividing the point cloud into vertical pillars rather than voxels. For each pillar, \textit{Pillar Feature Net} is applied to extract the point-level feature.} %Then 2d convolution network is adopted on the bird-eye-view feature map for object detection. %PointPillars is a trade-off between efficiency and performance.
    % \item \textit{PointRCNN \cite{shi2020points}} is a pure point cloud-based two-stages 3D object detector. For extract multi-scale features, the PointNet++ \cite{qi2017pointnet++} is taken as the backbone. First, the region proposal is generated with a binary foreground/background classifier in the first stage and then the proposal is refined by cropped points and features in the second stage.
    \item\textit{PV-RCNN \cite{shi2020pv}} is a hybrid point-voxel-based 3D object detector, which can utilize the advantages from both the point and voxel representations.
\end{enumerate}

\noindent\textbf{Implementation Details.} DeeplabV3+ \cite{deeplabv3plus2018} and Cylinder3D \cite{zhu2021cylindrical} are employed for 2D and 3D scene parsing respectively. More details, the DeeplabV3+ is pre-trained on Cityscape \footnote{\url{https://www.cityscapes-dataset.com}}, and the Cylinder3D is trained on KITTI point clouds by taking points in 3D ground trues bounding box as foreground annotation. For AAF module, $m = 4$, $C_1 = 64,C_2 = 128$, respectively. {The voxel size for PointPillars and SECOND are $0.16m \times 0.16m \times 4m$ and $0.05m \times 0.05m \times 0.1m$} respectively. In addition, both of the two baselines use the same optimization (e.g., AdamW) and learning strategies (e.g., one cycle) for all the experiments.
{In the DFF module, we set $C = 256$ and $C' = 512$ for \textit{SECOND} and \textit{PV-RCNN} framework and $C = 64$ and $C' = 384$ for \textit{PointPillars} network. The kernel and stride size are represented with $k$ and $s$ in Fig.\ref{fig:deep_feature_fusion}, respectively.}

%And all the experiments share the same settings with baseline, including voxel size, optimizer, and strategy of the learning rate, etc.
{The proposed approach is implemented with PaddlePaddle \cite{PaddlePaddle_2019} and all the methods are trained on NVIDIA Tesla V100 with 8 GPUs. The AdamW is taken as the optimizer and the one-cycle learning strategy is adopted for training the network. For \textit{SECOND} and \textit{PointPillars}, the batch size is 4 per GPU and the maximum learning rate is 0.003 while the bath size is 2 per GPU and the maximum learning rate is 0.001 for \textit{PV-RCNN}.}



 

\noindent\textbf{Quantitative Evaluation.} We illustrate the results on 3D detection and Bird's-eye view in \tabref{tab:kitti_3D_detection} and \tabref{tab:KITTI_BEV_detection} respectively. %More importantly, to verify the generalization ability, we have tested the proposed fusion strategy on three different baselines including voxel-based, pillar-based,hybrid point-voxel-based approaches.
%We can see more details on the tables. Especially, all the results in the tables are calculated by 40 recall positions. 
{From the table, we can clearly see that remarkable improvements have been achieved on the three baselines across all the categories.}
%The results show that our method achieved remarkably better mAP on all baselines.
Taking Pointpillars as an example, the proposed method has achieved 0.43\%, 6.65\%, 1.55\% points improvements on ``Car'', ``Pedestrian'' and ``Cyclist'' respectively. Interestingly, compared to ``Car'', ``Pedestrian'' and ``Cyclist'' give much more improvements by the fusion painting modules. 

%Interestingly, This phenomenon also appears in nuScenes dataset. And we will show more details and explain the contribution of different the module in ablation studies part.
\begin{table*}[ht!]
    \centering
    \Large
    % \renewcommand\arraystretch{1.1}
\resizebox{0.9\textwidth}{!}{

\begin{tabular}{ l| c| c| c| c c c c c c c c c c}
    \hline
    {\multirow{2}{*}{Methods}}  & 
    {\multirow{2}{*}{Modality}} & {\multirow{2}{*}{\textbf{NDS}(\%)}} & 
    {\multirow{2}{*}{\textbf{mAP}(\%)}} & 
    \multicolumn{10}{c}{\textbf{AP} (\%)} \\ 
    {} & {} & {} & {} & {Car} & {Truck} & {Bus} & {Trailer} & {Cons} & {Ped} & {Moto} & {Bicycle} & {T.C} & {Barrier} \\ \hline \hline
    PointPillars \cite{vora2020pointpainting} & L & 55.0 & 40.1 & 76.0 & 31.0 & 32.1 & 36.6 & 11.3 & 64.0 & 34.2 & 14.0 & 45.6 & 56.4 \\
    3DSSD \cite{yang20203dssd} & L  & 56.4 & 46.2 & 81.2  & 47.2  & 61.4  &  30.5 & 12.6 &  70.2 & 36.0  &  8.6 &  31.1 &  47.9 \\
    CBGS \cite{zhu2019class} & L & 63.3 & 52.8 & 81.1 & 48.5 & 54.9 & 42.9 & 10.5 & 80.1 & 51.5 & 22.3 & 70.9 & 65.7 \\
    HotSpotNet \cite{chen2020object} & L & 66.0 & 59.3 & 83.1  & 50.9 & 56.4  & 53.3  &  {23.0} &  81.3 & {63.5}  &  36.6 &  73.0 &  71.6 \\
    CVCNET\cite{chen2020every} & L & 66.6 & 58.2 & 82.6 & 49.5 & 59.4 & 51.1 & 16.2 & {83.0} & 61.8 & {38.8} & 69.7 & 69.7 \\
    CenterPoint \cite{yin2021center} & L & {67.3} & {60.3} & {85.2} & {53.5} & {63.6} & {56.0} & 20.0 & 54.6 & 59.5 & 30.7 & {78.4} & 71.1 \\
    PointPainting \cite{vora2020pointpainting} & L \& C & 58.1 & 46.4 & 77.9 & 35.8 & 36.2 & 37.3 & 15.8 & 73.3 & 41.5 & 24.1 & 62.4 & 60.2 \\
    3DCVF \cite{DBLP:conf/eccv/YooKKC20} & L \& C & 62.3 & 52.7 & 83.0 & 45.0 & 48.8 & 49.6 & 15.9 & 74.2 & 51.2 & 30.4 & 62.9 & 65.9 \\ \hline
    % Previous Version  & L \& C & 70.4 & 66.3 & 86.3 & 58.5 & 66.8 & 59.4 & 27.7 & 87.5 & 71.2  & 51.7 & 84.2 & 70.2 \\ 
    {Our proposed} & L \& C & \textbf{71.6} & \textbf{68.2} & \textbf{87.1} & \textbf{60.8} & \textbf{66.5} & \textbf{61.7} & \textbf{30.0} & \textbf{88.3} & \textbf{74.7} & \textbf{53.5} & \textbf{85.0} & \textbf{71.8}  \\  
    % Improvement $\uparrow$ & - & \textcolor{red}{\textbf{+1.20}} & \textcolor{red}{\textbf{+1.90}} & \textcolor{red}{+0.80} & \textcolor{red}{+2.3} & \textcolor{green}{-0.3} & \textcolor{red}{+2.3} & \textcolor{red}{+2.3} & \textcolor{red}{+0.8} & \textcolor{red}{+3.5} & \textcolor{red}{+1.8} &  \textcolor{red}{+0.8}&\textcolor{red}{+1.6} \\
    \hline
    \end{tabular}

}
\caption{Comparison with other SOTA methods on the nuScenes 3D object detection testing benchmark. ``L'' and ``C'' in the modality column represent LiDAR and Camera sensors respectively. For easy understanding, the highest score in each column is shown in bold font. To be clear, only the results with publications are listed here.}
\label{tab:test_tabel}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Detectors, Dataset and Implementation Details} \label{subsec:dataset}
\subsection{Evaluation on the nuScenes Dataset} \label{subsec:nuScenes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Evaluation resulst show that fusing Lidar and image information always yields significant gains over LIDAR-only based methods,as we showed in Table,all the classes detect accuracy has improved.
The nuScenes \cite{caesar2020nuscenes} is a recently released large-scale (with a total of 1,000 scenes) AD benchmark with different kinds of information including LiDAR point cloud, radar point, Camera images, and High Definition Maps, etc. For a fair comparison, the dataset has been divided into ``train'', ``val'', and ``test'' three subsets officially, which includes 700 scenes (28130 samples), 150 scenes (6019 samples), and 150 scenes (6008 samples) respectively. Objects are annotated in the LiDAR coordinate and projected into different sensors' coordinates with pre-calibrated intrinsic and extrinsic parameters. For the point clouds stream, only the keyframes (2fps) are annotated. With a 32 lines LiDAR scanner, each frame contains about {300,000} points for 360-degree viewpoint. For the object detection task, the obstacles have been categorized into 10 classes as ``car'', ``truck'', ``bicycle'' and ``pedestrian'' etc. Besides the point clouds, the corresponding RGB images are also provided for each keyframe, and for each keyframe, there are 6 cameras that can cover 360 fields of view.


\noindent\textbf{Evaluation Metrics.} The evaluation metric for nuScenes is totally different from KITTI and they propose to use mean Average Precision (mAP) and nuScenes detection score (NDS) as the main metrics. Different from the original mAP defined in \cite{everingham2010pascal}, nuScenes consider the BEV center distance with thresholds of \{0.5, 1, 2, 4\} meters, instead of the IoUs of bounding boxes. NDS is a weighted sum of mAP and other metric scores, such as average translation error (ATE) and average scale error (ASE). For more details about the evaluation metric please refer to \cite{caesar2020nuscenes}.

\noindent\textbf{Baselines.} We have integrated the proposed module on three different SOTA baselines to verify its effectiveness. Similar to the KITTI dataset, both the \textit{SECOND} and \textit{PointPillars} are employed and the other detector is \textit{CenterPoint} \cite{yin2021center}. which is the first anchor-free-based 3D object detector for LiDAR-based 3D object detection.  

%\begin{itemize}
%\item \textit{SECOND} \cite{yan2018second}, which is the first to employ the sparse convolution on the voxel-based 3D object detection task and the detection efficiency has been highly improved compared to previous work such as VoxelNet. 
%\item \textit{PointPillars} \cite{lang2019pointpillars}, which divides the point cloud into pillars and ``Pillar Feature Net'' is applied to each pillar for extracting the point feature. Then 2d convolution network has been adopted on the bird-eye-view feature map for object detection. PointPillars is a trade-off between efficiency and performance. 
%\item \textit{CenterPoint} \cite{yin2021center}, is the first anchor-free based 3D object detector which is very suitable for small object detection. 
%\end{itemize}

\noindent\textbf{Implementation Details} HTCNet \cite{chen2019hybrid} and Cylinder3D \cite{zhu2021cylindrical} are employed here for obtaining the 2D and 3D semantic segmentation results respectively. We used the HTCNet model trained on nuImages \footnote{\url{https://www.nuscenes.org/nuimages}} dataset directly for generating the semantic labels. For Cylinder3D, we train it directly on the nuScenes 3D object detection dataset while the point cloud semantic label is produced by taking the points inside each bounding box. In AAF module, $m = 11$, $C_1 = 64$ and  $C_2 = 128$ respectively. 
{In DFF module, $C = 256 $ and $C' = 512$ for \textit{SECOND} and \textit{CenterPoint} while $C = 64$ and $C' = 384$ for \textit{PointPillars}. The setting for kernel size $k$ and stride $s$ are given in Fig. \ref{fig:deep_feature_fusion} and same for all three detectors.} The voxel size for PointPillars, SECOND and CenterPoint are $0.2m \times 0.2m \times 8 m$, $0.1m \times 0.1m \times0.2m$ and $0.075m \times 0.075m \times 0.075m$, respectively. We use AdamW \cite{ loshchilov2019decoupled} as the optimizer with the max learning rate is 0.001. Following \cite{caesar2020nuscenes}, 10 previous LiDAR sweeps are stacked into the keyframe to make the point clouds more dense.

%\{For DFF module, taking SECOND framework in KITTI dataset as example. after 3d backbone, we get $C=256,C^{'}=512,W=200,H=176$. Here, we can adaptively choose the number of channel number. $Conv\_block1$ consists of several conv2d, $Conv(C,128,k=3,s=2)$ which present the number of input channel, out channel number is 256 and 128, kernal size and stride are 3 and 2 respectively. The meaning of k,s denotes that kernel size and stride, and x3 in the Table.\ref{fig:deep_feature_fusion} present three same parameters of conv2d but not share the weight. The letter $C^{'}$ is the output channel you want to change.}

%\xsqcomments{For DFF module, taking SECOND framework in KITTI dataset as example. after 3d backbone, we get $C=256,C^{'}=512,W=200,H=176$. Here, we can adaptively choose the number of channel number. $Conv\_block1$ consists of several conv2d, $Conv(C,128,k=3,s=2)$ which present the number of input channel, out channel number is 256 and 128, kernal size and stride are 3 and 2 respectively. The meaning of k,s denotes that kernal size and stride, and x3 in the Table.\ref{fig:deep_feature_fusion} present three same parameters of conv2d but not share the weight. The letter $C^{'}$ is the output channel you want to change.}

{All the baselines are trained on NVIDIA Tesla V100 (8 GPUs) with a batch size of 4 per GPU for 20 epochs. AdamW is taken as the optimizer and the one-cycle learning strategy is adopted for training the network with the maximum learning rate is 0.001.} 

%\xsqcomments{\textit{Training and inference Details:} Our MSF framework is trained on NVIDIA Tesla V100. And our method is coding in Pytorch framework. For KITTI dataset, we train the entire network on Pointpillar and SECOND with the batch size 4, learning rate 0.003, and PV-RCNN framework batch size is 2, learning rate is 0.001. All algorithms on KITTI dataset is trained 80 epochs. For nuScenes dataset, we train the entire network with batch size 4 for 20 epochs. the one-cycle learning rate strategy is adopted for the learning and the max learning rate is 0.001. And the optimizer is ADAM. } 



%\xsqcomments{\textit{Training and inference Details:} Our MSF framework is trained on NVIDIA Tesla V100. And our method is coding in Pytorch framework. For KITTI dataset, we train the entire network on Pointpillar and SECOND with the batch size 4, learning rate 0.003, and PV-RCNN framework batch size is 2, learning rate is 0.001. All algorithms on KITTI dataset is trained 80 epochs. For nuScenes dataset, we train the entire network with batch size 4 for 20 epochs. the one-cycle learning rate strategy is adopted for the learning and the max learning rate is 0.001. And the optimizer is ADAM. } 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent\textbf{Quantitative Evaluation.}  
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{The proposed framework has been evaluated on nuScenes benchmark for both ``val'' and ``test'' splits.} {The results of comparison with three baselines are given in Tab. \ref{tab:eval_on_nuscenes_val}. From this table, we can see that significant improvements have been achieved on both the $\text{mAP}$ and $\text{NDS}$ across all the three baselines. For the \textit{PointPillars}, the proposed module gives \textbf{8.93} and \textbf{18.29} points improvements on $\text{NDS}$ and $\text{mAP}$ respectively. For \textit{SECOND}, the two values are \textbf{5.65} and \textbf{11.76} respectively. Even for the strong baseline \textit{CenterPoint}, the proposed module can also give \textbf{5.09} and \textbf{9.32} points improvements.}
In addition, we also find that the {categories which share small sizes} such as ``Traffic Cone'', ``Moto'' and ``Bicycle'' have received more improvements compared to other categories. Taking ``Bicycle'' as an example, the $\text{mAP}$ has been improved by {36.46\%}, {49.41\%} and {26.49\%} compared to \textit{SECOND}, \textit{PointPillar} and \textit{Centerpoint} respectively. {This phenomenon can be explained as these categories with small sizes are hard to be recognized in point clouds because of a few LiDAR points on them. In this case, the semantic information from the 2D/3D parsing results is extremely helpful for improving 3D object detection performance. It should be emphasized that the result in Tab. \ref{tab:eval_on_nuscenes_val} without any Test Time Augmentation(TTA) strategies.}

%We can directly see the results of the experiments on different baselines in Tab. \ref{tab:eval_on_nuscenes_val} which has achieved great consistent\ improvements on both $\text{mAP}$ and $\text{NDS}$. Detailed results are given in the table. And in this table, we can obviously find that the proposed module gives more than 6.81 points improvements on $\text{mAP}$ and  3.31 points improvements on $\text{NDS}$ for the highest baseline of all. The improvements have reached 18.29 and 8.93 points for PointPillars method  on $\text{mAP}$ and $\text{NDS}$ respectively. In addition, we find that the category which has fewer point such as ``Traffic Cone'', ``Moto'' and ``Bicycle'' has received surprising improvements compared to other classes. For ``Bicycle'' category specifically, the AP has improved  {36.46\%}, {49.41\%} and {22.57\%} based on SECOND, PointPillar and Centerpoint respectively. Interestingly, all these categories are small objects which are hard to be detected because of a few LiDAR points on them. These verified that semantic information is helpful for 3D object detection task. Especially, the experiments here we share the same setting in the self environment, so the baseline figures may be subtle differences with the official.

To compare the proposed framework with other SOTA methods, we submit our results (adding fusion modules on \textit{CenterPoint}) on the nuScenes evaluation sever\footnote{\url{https://www.nuscenes.org/object-detection/}} for test split. The detailed results are given in Tab. \ref{tab:test_tabel}. From this table, we can find that the proposed method achieves the best performance on both the $\text{mAP}$ and $\text{NDS}$ scores. Compared to the baseline \textit{CenterPoint}, 4.3 and 7.9 points improvements have been achieved by adding our proposed fusion modules. For easy understanding, we have highlighted the best performances in bold in each column. It should be noted that the results in Tab. \ref{tab:test_tabel} the Test Time Augmentation(TTA) strategy including multiple flip and rotation operations is applied during the inference time which is 1.69 points higher than the origin method of ours.

 
 



==> Files/05_ablation_study.tex <==
\subsection{Ablation Studies} \label{subsec:ablation_study}

%\xsqcomments{In this part, we design several ablation experiments to analyze the contribution of different components for the final detection results. Specially, we have designed two series of experiments for nuScenes dataset. To be clear, we take the ``Semantic Score'' as the input for all the following experiments. Here, we just verify the different representations of 3D semantic information as example. }

{To verify the effectiveness of different modules, a series of ablation experiments have been designed to analyze the contribution of each component for the final detection results. Specially, three types of experiments are given as \textit{different semantic representations} and \textit{different fusion modules} and \textit{effectiveness of channel attention}.
}

\begin{table}[ht!]
\centering
\small
\renewcommand\arraystretch{1.1}
\resizebox{0.4\textwidth}{!}
{   
    \begin{tabular}{r | cccc}
    \hline
    $\textbf{Representations}$ & $\textbf{mAP }$ (\%) & $\textbf{NDS}$ (\%)  \\ \hline %\hline
    {PointPillar \cite{lang2019pointpillars}} & 43.46 & 57.50  \\ 
    {Semantic ID}    & 50.96 (+7.50)  & 60.69 (+3.19)   \\ 
    {Onehot Vector}   & 52.18 (+8.72)  & 61.59 (+4.09)   \\ 
    {Semantic Score}  & 53.10 (+9.64)  & 62.20 (+4.70)   \\ \hline
    \end{tabular}
}
\caption{Ablation studies on the nuScenes \cite{geiger2012we} dataset for fusing the semantic results with different representations.}
\label{tab:ablation_dif_semantic_reps}
\end{table}

\noindent\textbf{Different Semantic Representations.} First of all, we investigate the influence of the different semantic result representations on the final detection performance. Three different representations as ``Semantic ID'', ``Onehot Vector'' and ``Semantic Score'' are considered here. For ``Semantic ID'', the digital class ID is used directly and for the ``Semantic Score'', the predicted probability after the Softmax operation is used. In addition, to convert the semantic scores to a ``Onehot Vector'', we assign the class with the highest score as ``1'' and keep other classes as ``0''. Here, we just add the semantic feature to the original $(x, y, z)$ coordinates with concatenation operation and \textit{PointPillars} is taken as the baseline on nuScenes dataset due to its efficiency of model iteration. From the results in \tabref{tab:ablation_dif_semantic_reps}, we can easily find that the 3D semantic information can significantly boost the final object detection performance regardless of different representations. More specifically, the ``Semantic Score'' achieves the best performance among the three which gives 9.64 and 4.70 points improvements for $\textbf{mAP}$ and $\textbf{NDS}$ respectively. We guess that the semantic score can provide more information than the other two representations because it not only provides the class ID but also the confidence for all the classes.    

\iffalse
\begin{table}[ht!]
\centering
\resizebox{0.5\textwidth}{!}
{%
    \begin{tabular}{r | cccc}
    \hline
    $\textbf{Strategies}$ & $\textbf{Car} (Mod.)$ & $\textbf{Pedestrian}$ (Mod.) & $\textbf{Cyclist}$ (Mod.) \\ %\hline \hline
    {PointPillar \cite{lang2019pointpillars}} & 78.17 & 47.58 & 62.95  \\ 
    {Semantic ID.}    & 78.42(+0.25)   & 48.94(+1.36)  & 57.88(-5.07)  \\ 
    {Onehot Vector}    & 78.55(+0.35)  & 50.15(+2.57)   & 54.14(-8.81)  \\  
    {Semantic Score}  & 79.08(+0.91)   & 51.41(+3.93)   & 61.25(-1.70)   \\ \hline
    \end{tabular}
}
\caption{Ablation studies on the public KITTI \cite{geiger2012we} dataset. The way use 3D semantic info. To be clear, only the results of the ``Moderate'' category have been given and the mAP represents the mean AP of ``Car'', ``Pedestrian'' and ``Cyclist''.}
\label{tab:ablation_kitti_table}
\end{table}
\fi


\noindent\textbf{Different Fusion Modules.} We also execute different experiments to analyze the performances of each fusion module on both KITTI and nuScene  dataset. The \textit{SECOND} is chosen as the baseline for KITTI while all the three detectors are verified on nuScene. 
%Specifically, all the experiments are executed on the validation split and the settings are kept the same as previous subsections. 
The results are given in \tabref{tab:ablation_kitti_table} and \tabref{tab:ablation_nuScene_table} for KITTI and nuScenes respectively. To be clear, the ``3D Sem'' and ``2D Sem.'' represent the 2D and 3D parsing results. ``AAF'' represents the fusion of the 2D and 3D semantic information with the proposed adaptive attention module and the ``AAF + DFF'' represents the module with both the two fusion strategies.

\begin{table}[t]
\centering
\small
% \renewcommand\arraystretch{1.1}
\resizebox{0.5\textwidth}{!}
{%
    \begin{tabular}{r | ccc|l}
    \hline
\multirow{2}{*}{Strategies} & \multicolumn{3}{c|}{AP(\%)}  & \multirow{2}{*}{mAP(\%)} \\
                            & \multicolumn{1}{l}{Car(Mod.)} & \multicolumn{1}{l}{Ped.(Mod.)}   & \multicolumn{1}{l|}{Cyc.(Mod.)}  &  \\ \hline
    {SECOND \cite{yan2018second}} & 88.99 & 56.21 & 70.65 & 71.95 \\ %\hline 
    {3D Sem.}             & + 0.81  &  + 0.70  &  + 0.63  & + 0.71  \\ 
    {2D Sem.}    &  + 1.09 &  + 1.35  &  + 1.20  &  + 1.41  \\ 
    {AAF}  & + 1.62   &  + 1.78  &  + 1.91  & + 1.77  \\ 
    {AAF \& DFF} & + 2.63   &  + 3.45  &  + 2.63  &  + 2.90 \\ \hline
    \end{tabular}
}
\caption{Evaluation of ablation studies on the public KITTI \cite{geiger2012we} dataset. Similar to PointPainting \cite{vora2020pointpainting}, we provide the 2D BEV detection here. To be clear, only the results of ``Mod'' have been given and \textbf{mAP} is the average mean of all the three categories.}
\label{tab:ablation_kitti_table}
\end{table}


\begin{table}[ht!]
\centering
\setlength{\tabcolsep}{2pt}
\renewcommand\arraystretch{1.1}
\resizebox{0.5\textwidth}{!}
{%
    \begin{tabular}{r | cc | cc |cc}
    \hline
    \multicolumn{1}{r|}{\multirow{2}{*}{\textbf{Strategies}}} & 
    \multicolumn{2}{c|}{\textbf{SECOND}}   & 
    \multicolumn{2}{c|}{\textbf{PointPillars}} & 
    \multicolumn{2}{c}{\textbf{CenterPoint}}  \\ %\cline{2-14} 
   {}  & \textbf{mAP}(\%) & \textbf{NDS}(\%) &  \textbf{mAP}(\%) & \textbf{NDS}(\%)& \textbf{mAP}(\%)& \textbf{NDS}(\%) 
   \\ \hline  %\hline
    {SECOND}         &  50.85 &  61.96 &   43.46 &  57.50    &  56.53 & 64.82\\ %\hline
    {3D Sem.}        &   + 3.60&   + 1.45  & + 8.72  &  + 4.09 & + 4.59 & + 1.86 \\ 
   {2D Sem.}         &   + 8.55&   + 4.07  &  +15.64   &+ 7.55    & + 6.28 & + 3.67 \\ 
    {AAF}   & + 11.30  &  + 5.45   &  +17.31   & + 8.54   & + 8.46& + 4.56 \\ 
   {AAF \& DFF}  &  + 11.76 &  + 5.65   &  +  18.19  & + 8.93     & + 9.32 & + 5.09\\ \hline
    \end{tabular}
}
\caption{Ablation studies for different fusion strategies on the nuScenes benchmark. The first row is the performance of the baseline method and the following values are the gains obtained by adding different modules.}
\label{tab:ablation_nuScene_table}
\end{table}

In \tabref{tab:ablation_kitti_table}, the first row is the performance of the baseline method and the following values are the gains obtained by adding different modules. From the table, we can obviously find that all the modules give positive effects on all three categories for the final detection results. For all the categories, the proposed modules give 2.9 points improvements averagely and ``Pedestrian'' achieves the most gain which achieves 3.45 points. Furthermore, we find that deep fusion gives the most improvements compared to the other three modules in this dataset.   

\tabref{tab:ablation_nuScene_table} gives the results on the nuScenes dataset. 
{To be clear, a boosted version of baseline is presented here than in \cite{xu2021fusionpainting} by fixing the sync-bn issue in the source code.} 
From this table, we can see that both the 2D and 3D {semantic information} can significantly boost the performances while the 2D information provide more improvements than the 3D information. This phenomenon can be explained as that the 2D texture information can highly benefit the categories classification results which is very important for the final \textbf{mAP} computation. In addition, by giving the 2D information, the recall ability can be improved especially for objects in long distance with a few scanned points. In other words, the advantage for 3D semantic information is that the point clouds can well handle the occlusion among objects which are very common in AD scenarios which is hard to deal with in 2D. After fusion, all the detectors achieve much better performances than only one semantic information (2D or 3D).

Furthermore, a deep fusion module is also proposed to aggregate the backbone features to further improve the performance. From the Tab. \tabref{tab:ablation_kitti_table} and \tabref{tab:ablation_nuScene_table}, we find that the deep fusion module can slightly improve the results for all three baseline detectors. Interestingly, compared to the \textit{SECOND} and \textit{PointPillars}, \textit{CenterPoint} gives much better performance by adding the deep fusion module. This can be explained that the large deep backbone network in \textit{CenterPoint} gives much deeper features that are more suitable for the proposed deep feature fusion module. 

\iffalse
\begin{table}[ht!]
\centering
\resizebox{0.5\textwidth}{!}
{%
    \begin{tabular}{r | cc | cc }
    \hline
    \multicolumn{1}{r|}{\multirow{2}{*}{\textbf{Strategies}}} & 
    \multicolumn{2}{c|}{\textbf{SECOND}} & 
    \multicolumn{2}{c}{\textbf{CenterPoint}}  \\ %\cline{2-14} 
   {}  & \textbf{NDS}(\%) & \textbf{mAP}(\%) &  \textbf{NDS}(\%) & \textbf{mAP}(\%)  \\ \hline  %\hline
    {Baselines}  &  50.85 &  61.96 & 59.04 & 66.60\\ %\hline
    {Without CA.} & 52.24(\R{+1.39})& 63.18(\R{+0.85}) &67.45(\R{+0.8}) &59.84(\R{+1.08}) \\ 
   {Baseline with DFF.} &52.96(\R{+2.11})&63.75(\R{+1.79}) &67.84(\R{+1.24}) &60.20(\R{+1.16}) \\ \hline
    \end{tabular}
}
\caption{Ablation with/without channel attention on nuScenes dataset.}
\label{tab:ablation_channel_attention_nuscenes}
\end{table}
\fi

 

\begin{table}[t]
\centering
\renewcommand\arraystretch{1.1}
\setlength{\tabcolsep}{1pt}
\resizebox{0.5\textwidth}{!}
{%
\begin{tabular}{r|ccc|c} 
\hline
\multirow{2}{*}{\textbf{Strategies}} & \multicolumn{3}{c|}{\textbf{AP(\%)}}                                                                            & \multirow{2}{*}{\textbf{mAP(\%)}}        \\
                            & \multicolumn{1}{l}{Car(Mod.)}    & \multicolumn{1}{l}{Ped.(Mod.)}   & \multicolumn{1}{l|}{Cyc.(Mod.)}  &                                 \\ 
\hline
SECOND                      & ~88.99~                          & 56.21                            & 70.65                            & 71.95                           \\
One scale CA                & ~89.68 (\textcolor{red}{+0.69})~ & 57.77 (\textcolor{red}{+1.56})   & ~71.39 (\textcolor{red}{+0.74})~ & 73.70 (\textcolor{red}{+1.75})  \\
Multi-scale CA              & 90.22 (\textcolor{red}{+1.23})   & ~58.11 (\textcolor{red}{+1.90})~ & ~71.77 (\textcolor{red}{+1.12})~ & 74.41 (\textcolor{red}{+2.46})  \\
\hline
\end{tabular}
}
\caption{Ablation with/without multi-scale channel attention (CA) on KITTI dataset. The meaning of \textit{one-scale CA} is we just use $F_{R}^{L}$ to the \textit{CA} module. And multi-scale denote that we use both  fused $F_{R}^{L}$ and $F_{R}^{S}$ feature to the next module.}
\label{tab:ablation_channel_attention_kitti}
\end{table}


\noindent\textbf{Effectiveness of Multi-scale CA.} {In addition, a small experiment is also designed for testing the effectiveness of multi-scale attention in the DFF module. \textit{SECOND} is taken as the baseline and tested on the KITTI dataset. From the results given in Tab. \ref{tab:ablation_channel_attention_kitti}, we can see that by employing the one-scale features, the \textbf{mAP} has been improved by 1.75 points compared to the baseline. By adding the multi-scale operation, additional 0.71 points improvements can be further obtained.}


%\xsqcomments{And in order to verify the contribution of different part of DFF module, we do more experiments with different baseline and dataset as Tab.\ref{tab:ablation_channel_attention_nuscenes} and Tab.\ref{tab:ablation_channel_attention_kitti} shown. We can directly see that both of the network which fuse different receptive fields and channel attention module has positive effective for the final detection results. Taking Tab.\ref{tab:ablation_channel_attention_nuscenes} as example. The baseline of SECOND imporved 2.11 NDS by using DFF module while without channel attention module gained 1.39 point. This phenomenon indicate that the channel attention module in the DFF can take 0.72 NDS point improvement.}

\iffalse
\begin{table}[ht!]
\centering
\resizebox{0.5\textwidth}{!}
{%
    \begin{tabular}{r | cccc}
    \hline
    $\textbf{Strategies}$ & $\textbf{Car} (Mod.)$ & $\textbf{Pedestrian}$ (Mod.) & $\textbf{Cyclist}$ (Mod.) & $\textbf{mAP }$ (\%) \\ \hline \hline
    {PointPillar \cite{lang2019pointpillars}} &  &  &  &  \\ 
    {Semantic ID.}             &   &   &    &   \\ 
    {Onehot Vector}    &   &    &    &    \\ 
    {Semantic Score}  &    &    &    &   \\ \hline
    \end{tabular}
}
\caption{Ablation studies on the public KITTI \cite{geiger2012we} dataset. The way use 3D semantic info. To be clear, only the results of the ``Moderate'' category have been given and the mAP represents the mean AP of ``Car'', ``Pedestrian'' and ``Cyclist''.}
\label{tab:ablation_kitti_table}
\end{table}
\begin{table}[ht!]
\centering
\resizebox{0.35\textwidth}{!}
{%
    \begin{tabular}{r | cccc}
    \hline
    $\textbf{Strategies}$ & $\textbf{mAP }$ (\%) & $\textbf{NDS}$ (\%)  \\ \hline \hline
    {PointPillar \cite{lang2019pointpillars}} & 44.46 & 57.50  \\ 
    {Semantic ID.}     & 50.96 (+7.50)  & 60.69 (+3.19)   \\ 
    {Onehot Vector}   &  52.18 (+8.72) &  61.59 (+4.09)   \\ 
    {Semantic Score}  & 53.10 (+9.64)   &  62.20 (+4.70)    \\ \hline
    \end{tabular}
}
\caption{Ablation studies on the public nuScenes \cite{geiger2012we} dataset for different semantic representations.   }
\label{tab:ablation_dif_semantic_reps}
\end{table}
\fi


\iffalse
\begin{table}[ht!]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l | c c c c l l }
\hline
\textbf{Baselines} &  \textbf{3D-Sem} & \textbf{2D-Sem} & \textbf{ShallowFusion} & \textbf{DeepFusion} & \textbf{mAP(\%)} & \textbf{NDS(\%)} \\ \hline
\multirow{4}{*}{\textbf{SECOND}}   & -- & -- & -- & -- &50.85 (baseline) &61.96 (baseline)  \\
                 &\checkmark  &  & & &54.45 (\textcolor{red}{+3.60})  &63.41 (\textcolor{red}{+1.45})  \\
                  &  & \checkmark & & &59.40 (\textcolor{red}{+8.55}) &66.03 (\textcolor{red}{+4.07})  \\
                 % &\checkmark & \checkmark&  &62.15(+11.3)  & 67.41(+5.45)  \\
                  & \checkmark &  \checkmark &  \checkmark & &62.15 (\textcolor{red}{+11.30})  & 67.41 (\textcolor{red}{+5.45})  \\ 
                   & \checkmark & \checkmark & \checkmark & \checkmark &62.86 (\textcolor{red}{+12.01})  & 68.05 (\textcolor{red}{+6.09}) \\ \hline
\multirow{4}{*}{\textbf{PointPillars}} & -- & --  & -- & -- &43.46 (baseline) &57.50 (baseline)   \\
                      & \checkmark &  &  & &52.18 (\textcolor{red}{+8.72})  &61.59 (\textcolor{red}{+4.09})   \\
                     &  & \checkmark  & &  &59.10 (\textcolor{red}{+15.64}) & 65.05 (\textcolor{red}{+7.55})  \\
                  %   & \checkmark & \checkmark &  &60.77 (+17.31) &66.04 (+8.54)  \\ 
                    & \checkmark &  \checkmark &  \checkmark & & 60.77 (\textcolor{red}{+17.31}) &66.04 (\textcolor{red}{+8.54})   \\ 
                     & \checkmark & \checkmark & \checkmark & \checkmark &61.58 (\textcolor{red}{+18.12})  & 66.78 (\textcolor{red}{+9.28}) \\ \hline
\multirow{4}{*}{\textbf{CenterPoint}} & -- & --  & -- & -- &59.04 (baseline) & 66.60 (baseline) \\
        & \checkmark &  & & & 61.12 (\textcolor{red}{+2.08})  &67.68 (\textcolor{red}{+1.08})   \\
            &  & \checkmark &  & & 62.81 (\textcolor{red}{+3.77}) & 68.49 (\textcolor{red}{+1.89})\\
        %& \checkmark  & \checkmark  &   & 61.65(+10.49)  & 65.58(+5.29)  \\
         & \checkmark & \checkmark & \checkmark & &64.99 (\textcolor{red}{+5.95})  & 69.38 (\textcolor{red}{+2.78}) \\ 
        & \checkmark & \checkmark & \checkmark & \checkmark &65.85 (\textcolor{red}{+6.81})  & 69.91 (\textcolor{red}{+3.31}) \\ \hline
        
\multirow{1}{*}{\textbf{CenterPoint*}} &\checkmark  &\checkmark  &\checkmark  &\checkmark&67.84 (\textcolor{red}{+8.80}) & 71.64 (\textcolor{red}{+5.04}) 

\\ \hline
\end{tabular}
}
\caption{An ablation study for different fusion strategies. ``Att-Mod'' is short for Adaptive Attention Module, ``3D-P'' and ``2D-P'' are short for ``3D Painting Module'' and ``2D Painting Module'', respectively. Especially, CenterPoint* means Centerpoint with Double Flip and DCN. }

\label{tab:ablation_table}
\end{table}
\fi 

\iffalse
\begin{table}[ht!]
\centering
\resizebox{0.4\textwidth}{!}
{%
\begin{tabular}{|l|c|c|}
\hline
 & PointPillars (ms) & SECOND (ms) \\ \hline
Baseline & 53.5 & 108.2 \\ \hline
+3D Sem & 56.5\textcolor{red}{(+3.0)} & 108.7\textcolor{red}{(+0.5)} \\ \hline
+2D Sem & 56.9\textcolor{red}{(+3.4)} & 108.4\textcolor{red}{(+0.2)} \\ \hline
+AAF+DFF & 62.5\textcolor{red}{(+9.0)} & 113.3\textcolor{red}{(+4.6)} \\ \hline
\end{tabular}
}
\caption{Running time of differ modules. Here, +3D Sem, +2D Sem, +AAF+DFF denote the inference time of use PointCloud segmentation, image semantic segmentataion and both of two type segmentaion and AAF \& DFF module. }
\label{tab:differ running time}
\end{table}
\\
\begin{table}[ht!]
\centering
\resizebox{0.4\textwidth}{!}
{%
\begin{tabular}{|c|c|c|c|}
\hline
Type & 2D Sem & 3D Sem & Projection \\ \hline
Time(ms) & 32ms & 140ms & 3ms \\ \hline
\end{tabular}
}
\caption{The type of 2D Sem and 3D Sem denote that the time of we got 2D semantic segmentation and 3D semantic segmentation respectively. And the Projection is the time of project pointcloud on semantic image to get the score of prediction result}
\label{tab:seg time}
\end{table}
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{\subsection{Computation Time}} \label{subsec:comp_time}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht!]
\centering
\setlength{\tabcolsep}{5pt}
\renewcommand\arraystretch{1.1}
\resizebox{0.35\textwidth}{!}
{   
    \begin{tabular}{r | cccc}
    \hline
    $\textbf{Types}$ & $\textbf{PointPillars }$ & $\textbf{SECOND}$ \\ \hline 
    {Baseline}      & 53.5 (ms) & 108.2 (ms) \\
    {+3D Sem}       & +3.0 (ms) & +0.5 (ms)    \\ 
    {+2D Sem}       & +3.4 (ms) & +0.2 (ms)    \\ 
    {The Proposed}   & 62.5 (ms) & 113.3 (ms)   \\ \hline
    \end{tabular}
}
\caption{Inference time of different modules. Here, \textit{+3D Sem} and \textit{+2D Sem} denote the time of adding 3D/2D semantic information to input data. \textit{The Proposed} denotes the proposed framework with the modules including two types of semantic information and \textit{AAF} \& \textit{DFF} modules.}
\label{tab:inference_time}
\end{table}


\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.975\textwidth]{Figs/det_res.pdf}
	\centering
	\caption{Visualization of detection results with Open3d \cite{zhou2018open3d}, where (a) is the ground-truth, (b) is the baseline method based on only point cloud, (c), (d) and (e) are the detection results based on the 2D semantic, 3D semantic and fusion semantic information, respectively. Especially, the yellow and red dash ellipses show some false positive and false negative detection. For nuScenes dataset, the baseline detector used here is CenterPoint, and for KITTI is SECOND.} %	 
	\label{Fig:detection result}
\end{figure*}

Besides the performance, the computation time is also very important. Here, we test the computation time of each module based on the {\textit{PointPillars} and \textit{SECOND} on the KITTI dataset in \tabref{tab:inference_time}.} For a single Nvidia V100 GPU, the \textit{PointPillars} takes 53.5 ms per frame. By adding the 2D and 3D semantic information, the inference time increases 3.0 ms and 3.4 ms respectively while the time increases about 9 ms by adding two types semantic information and the AFF \& DFF modules. The inference time for \textit{SECOND} is given at the right column of \tabref{tab:inference_time}. Compared with the baseline, the 2D/3D semantic segmentation information gives nearly no extra computational burden. We explain this phenomenon as that in \textit{SECOND} the simple \textit{mean} operation is employed for extracting the features for each voxel and the computation time of this operation will not change too much with the increasing of the feature dimension. For \textit{PointPillars}, the MPL is employed for feature extracting in each pillar, therefore the computation time will increase largely with the increasing of the feature dimension.

{In addition, we also record the time used for obtaining the 2D/3D semantic results. For Deeplab V3+, the inference time is about 32 ms per frame while for Cylinder3D, it takes about 140 ms per frame. Furthermore, the re-projection of 2D image to 3D point clouds also takes about 3 ms for each frame. The almost time consuming here are 2D/3D point clouds segmentation operations. But in the practical using there just need a extra segmentation head after detection network backbone. In other words, multi-head is needed here for both detection and segmentation task. These just taking few milliseconds when using model inference acceleration operation, like C++ inference library TensorRT.}
\\
%\xsqcomments{\textbf{Running Time}: The experiments verify the effective of the MSF moudle which get huge improvement base on the baseline. Here we also make more expeiments about time efficiency as Tab.\ref{tab:differ running time} and Tab.\ref{tab:seg time}. And in the Table.\ref{tab:differ running time}, there has less than 1 millisecond increased when add 3D Semantic and 2D Semantic infomation to input date in SECOND baseline.
%The running time increased 4.6 millisecond even though we both add AFF and DFF module to the framework. The results clear that the parts of network we proposed in the framework just increase a few time. But here we just static the time after pointcloud got 2D image segmentation or 3D segmentation results and send it to the framework in the Table.\ref{tab:differ running time}. The most time in the network are spend on getting 2D image and 3D pointcloud segmentation results. We can find that the inference time of getting 2D semantic segmentation results by using DeeplabV3+ network is about 32ms, the time of getting 3D semantic segmentation results is 140ms which uses Cylinder3D network. After we get 2D semantic image, we have to project pointcloud onto semantic image to get each point category information, total time of projection process is approximately 3ms. We can directly find all details in the Tabel.\ref{tab:seg time} and the time is test on KITTI dataset..}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Qualitative Detection Results}\label{sub:Qualitative_Res}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We show some qualitative detection results on nuScenes and KITTI dataset in \figref{Fig:detection result} in which \figref{Fig:detection result} (a) is the ground truth, (b), (c), and (d) are the detect result of baseline (CenterPoint) without any extra information, with 2D and 3D semantic information respectively and (e) is final results with all the fusion modules. From these figures, we can easily find that there is some false positive detection caused by the frustum blurring effect in 2D painting, while the 3D {semantic results} give a relatively clear boundary of the object but provides some worse class classification. More importantly, the proposed framework which combines both the two complementary information from 2D and 3D segmentation can give much more accurate detection results.


==> Files/back_up05_ablation_study_backup.tex <==
\subsection{Ablation Studies} \label{subsec:ablation_study}

In this part, we design several ablation experiments to analyze the contribution of different components for the final detection results. Specially, we have designed two series of experiments for both the KITTI and nuScenes dataset respectively. 




\textbf{KITTI Benchmark}: we choose the SECOND detector for the ablation study on KITTI benchmark. 
  

\begin{table}[ht!]
\centering
\resizebox{0.5\textwidth}{!}
{%
    \begin{tabular}{r | cccc}
    \hline
    $\textbf{Strategies}$ & $\textbf{Car} (Mod.)$ & $\textbf{Pedestrian}$ (Mod.) & $\textbf{Cyclist}$ (Mod.) & $\textbf{mAP }$ (\%) \\ \hline \hline
    {SECOND \cite{yan2018second}} & 88.99 & 56.21 & 70.65 & 71.95 \\ 
    {3D Sem.}             & + 0.81  &  + 0.70  &  + 0.63  & + 0.71  \\ 
    { 2D Sem.}    &  + 1.09 &  + 1.35  &  + 1.20  &  + 1.41  \\ 
    { Shallow Fusion}  & + 1.62   &  + 1.78  &  + 1.91  & + 1.77  \\ 
    { Deep Fusion } & + 2.63   &  + 3.45  &  + 2.63  &  + 2.90 \\ \hline
    \end{tabular}
}
\caption{Ablation studies on the public KITTI \cite{geiger2012we} dataset. Here, we take the SECOND \cite{yan2018second} as the baseline method. Similar to PointPainting \cite{vora2020pointpainting}, we provide the detection results on the Bird's-eye view here. To be clear, only the results of the ``Moderate'' category have been given and the mAP represents the mean AP of ``Car'', ``Pedestrian'' and ``Cyclist''.}
\label{tab:ablation_kitti_table}
\end{table}


\textbf{nuScenes Benchmark}: three different detectors have been employed for ablation here. The experimental results are given in \tabref{tab:ablation_nuScene_table}.

\begin{table}[ht!]
\centering
\resizebox{0.5\textwidth}{!}
{%
    \begin{tabular}{r | cc | cc |cc}
    \hline
    \multicolumn{1}{r|}{\multirow{2}{*}{\textbf{Strategies}}} & 
    \multicolumn{2}{c|}{\textbf{SECOND}}   & 
    \multicolumn{2}{c|}{\textbf{PointPillars}} & 
    \multicolumn{2}{c}{\textbf{CenterPoint}}  \\ %\cline{2-14} 
   {}  & \textbf{mAP} (\%) & \textbf{NDS} (\%) &  \textbf{mAP} (\%) & \textbf{NDS} (\%) & \textbf{mAP} (\%) & \textbf{NDS} (\%)  
   \\ \hline  \hline
    {Baseline}         &  50.85 &  61.96 &   43.46 &  57.50    &  59.04 & 66.60\\ 
    {3D Sem.}          &   + 3.60&   + 1.45  & + 8.72  &  + 4.09 & + 0.84 & + 0.58 \\ 
    {2D Sem.}          &   + 8.55&   + 4.07  &  + 15.64   &+ 7.55    & + 7.29& + 3.69 \\ 
    { ShallowFusion}   & + 11.30  &  + 5.45   &  + 17.31   & + 8.54   & + 10.00& + 5.86 \\ 
    { DeepFusion }     &  + 12.01 &  + 6.09   &  + 18.12  & + 9.28     & +xxxxx & + xxxxx\\ \hline
    \end{tabular}
}
\caption{An ablation study for different fusion strategies. ``Att-Mod'' is short for Adaptive Attention Module, ``3D-P'' and ``2D-P'' are short for ``3D Painting Module'' and ``2D Painting Module'', respectively. Especially, CenterPoint* means Centerpoint with Double Flip and DCN.}
\label{tab:ablation_nuScene_table}
\end{table}

For Second and PointPillars 3D detector we trained and evaluated with whole dataset,we can see that both of 3D and 2D segmentation information has clearly improved the detect accuracy as showed as Tabel.\ref{tab:ablation_table}(1th and 2th row),Pointpillar received largest mAP(+17.31) and NDS(+8.54) imporved compare with baseline,
while Centerpoint achieved that mAP(+10.49) and NDS(+5.29) imporved with quarter of the training split dataset and eval with whole dataset,Specilly we trained all the model with same config,with 8GPU and 4 batchsize, so the baseline maybe subtle differences between our experiment and official figures.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
To verify the effectiveness of different modules, a series of ablation studies have been designed here. All the experiments are executed on the validation split and the settings keep the same as in Sec. \ref{subsec:dataset}. All the results are given in Tab. \ref{tab:ablation_table}, from where we could figure out the impact of each module. 

As demonstrated in Tab. \ref{tab:ablation_table}, 3D semantic segmentation information alone contributes about 9.81\% mAP and 3.92\% NDS averagely, while 2D semantic segmentation information contributes about 21.90\% and 8.46\% averagely. The higher improvement from 2D semantic information benefit from the better recall ability especially for objects in the distance where the point cloud is very sparse. The advantage for 3D semantic information is that the point clouds can well handle the occlusion among objects which is very common and hard to deal in 2D. But the most improvement comes from the combination of 3D Painting, 2D Painting and Adaptive Attention Module, 26.58\% mAP and 10.90\% averagely from 3 detectors we used.

\begin{table}[ht!]
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l | c c c c l l }
\hline
\textbf{Baselines} &  \textbf{3D-Sem} & \textbf{2D-Sem} & \textbf{ShallowFusion} & \textbf{DeepFusion} & \textbf{mAP(\%)} & \textbf{NDS(\%)} \\ \hline
\multirow{4}{*}{\textbf{SECOND}}   & -- & -- & -- & -- &50.85 (baseline) &61.96 (baseline)  \\
                 &\checkmark  &  & & &54.45 (\textcolor{red}{+3.60})  &63.41 (\textcolor{red}{+1.45})  \\
                  &  & \checkmark & & &59.40 (\textcolor{red}{+8.55}) &66.03 (\textcolor{red}{+4.07})  \\
                 % &\checkmark & \checkmark&  &62.15(+11.3)  & 67.41(+5.45)  \\
                  & \checkmark &  \checkmark &  \checkmark & &62.15 (\textcolor{red}{+11.30})  & 67.41 (\textcolor{red}{+5.45})  \\ 
                   & \checkmark & \checkmark & \checkmark & \checkmark &62.86 (\textcolor{red}{+12.01})  & 68.05 (\textcolor{red}{+6.09}) \\ \hline
\multirow{4}{*}{\textbf{PointPilars}} & -- & --  & -- & -- &43.46 (baseline) &57.50 (baseline)   \\
                      & \checkmark &  &  & &52.18 (\textcolor{red}{+8.72})  &61.59 (\textcolor{red}{+4.09})   \\
                     &  & \checkmark  & &  &59.10 (\textcolor{red}{+15.64}) & 65.05 (\textcolor{red}{+7.55})  \\
                  %   & \checkmark & \checkmark &  &60.77 (+17.31) &66.04 (+8.54)  \\ 
                    & \checkmark &  \checkmark &  \checkmark & & 60.77 (\textcolor{red}{+17.31}) &66.04 (\textcolor{red}{+8.54})   \\ 
                     & \checkmark & \checkmark & \checkmark & \checkmark &61.58 (\textcolor{red}{+18.12})  & 66.78 (\textcolor{red}{+9.28}) \\ \hline
\multirow{4}{*}{\textbf{CenterPoint}} & -- & --  & -- & -- &59.04 (baseline) & 66.60 (baseline) \\
        & \checkmark &  & & & 61.12 (\textcolor{red}{+0.84})  &67.68 (\textcolor{red}{+0.58})   \\
            &  & \checkmark &  & & 61.12 (\textcolor{red}{+7.29}) & 67.68 (\textcolor{red}{+3.69})\\
        %& \checkmark  & \checkmark  &   & 61.65(+10.49)  & 65.58(+5.29)  \\
         & \checkmark & \checkmark & \checkmark & &64.89 (\textcolor{red}{+10.00})  & 69.38 (\textcolor{red}{+5.86}) \\ 
        & \checkmark & \checkmark & \checkmark & \checkmark &65.85 (\textcolor{red}{+10.00})  & 69.91 (\textcolor{red}{+5.86}) \\ \hline
        
%\multirow{1}{*}{\textbf{CenterPoint*}} &\checkmark  &\checkmark  &\checkmark  &\checkmark&67.84 (\textcolor{red}{+8.80}) & 71.64 (\textcolor{red}{+5.04}) 

\\ \hline
\end{tabular}
}
\caption{An ablation study for different fusion strategies. ``Att-Mod'' is short for Adaptive Attention Module, ``3D-P'' and ``2D-P'' are short for ``3D Painting Module'' and ``2D Painting Module'', respectively. Especially, CenterPoint* means Centerpoint with Double Flip and DCN. }

\label{tab:ablation_table}
\end{table}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Qualitative Results on KITTI and nuScenes Dataset}\label{sub:Qualitative_Res}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

More qualitative detection results are illustrated in Fig. \ref{Fig:detection result}. Fig. \ref{Fig:detection result} (a) shows the annotated ground truth, (b) is the detection results for CenterPoint based on raw point cloud without using any painting strategy. (c) and (d) show the detection results with 2D painted and 3D painted point clouds, respectively, while (e) is the results based on our proposed framework. 
As shown in the figure, there are false positive detection results caused 2D painting due to frustum blurring effect, while 3D painting method produces worse foreground class segmentation compared to  2D image segmentation. Instead, our FusionPainting can combine two complementary information from 2D and 3D segmentation, and detect objects more accurately.

\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.975\textwidth]{FusionPainting/TITS/Figs/results_rviz.pdf}
	\centering
	\caption{Visualization of detection results, where (a) is the ground-truth, (b) is the detection results based on raw point cloud, (c), (d) and (e) are the detection results based on the projected points with 2D semantic information, 3D semantic information and fusion semantic information, respectively. Especially, the yellow and red dash ellipses show some of the false and missed detection, respectively. The baseline detector used here is CenterPoint \cite{yin2020center}.} %	 
	\label{Fig:detection result}
\end{figure*}



==> Files/back_up_04_experiments_backup.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Results} \label{sec:experiments}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To verify the effectiveness of our proposed framework, we evaluate it on two the large-scale autonomous driving 3D object detection dataset as KITTI \cite{geiger2012we} and nuScenes \cite{nuscenes2019}. Furthermore, we also evaluate the proposed modules on different kinds of 3D detectors for verifying their generalizability, such as SECOND \cite{yan2018second}, PointPilars \cite{lang2019pointpillars}, PointRCNN \cite{shi2019pointrcnn} and PVRCNN \cite{shi2020pv} etc.

 
 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation on KITTI Dataset} \label{subsec:eval_kitti}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We test the proposed framework on the KITTI dataset first. 

\textit{KITTI \cite{geiger2012we}} as one of the most popular benchmarks for 3D object detection in AD, it contains 7481 samples for training and 7518 samples for testing. The objects in each class are divided into three difficulty levels as ``easy'', ``moderate'', and ``hard'', according to the object size, the occlusion ratio, and the truncation level. Since the ground truth annotations of the test samples are not available and the access to the test server is limited, we follow the idea in~\cite{chen2017multi} and split the source training data into training and validation where each set contains 3712 and 3769 samples respectively. In this dataset, both the point cloud and the RGB image have been provided. In addition, both the intrinsic camera parameters and extrinsic transformation parameters between different sensors have been well-calibrated. For the object detection task, multiple stereo frames have been provided while only a single image from the left camera at the current frame is used in our approach.

\textit{Evaluation Metrics:} we follow the metrics provided by the official KITTI benchmark for comparison here. Specifically, for ``Car'' class, we use the metric $\textbf{AP}_\text{Car}$\textbf{70} for all the detection results. $\textbf{AP}_\text{Car}$\textbf{70} means that only the samples in which the overlay of bounding box with ground truth is more than 70\% are considered as positive. While the threshold for ``Pedestrian'' class is 0.5 (e.g., $\textbf{AP}_\text{Ped}$\textbf{50}) due to its smaller size. Similar to \cite{vora2020pointpainting}, the average AP (mAP) of three Classes for ``Moderate'' is also taken as an indicator for evaluating the average performance on all three classes. 

For KITTI dataset, four different types of baselines have been evaluated here which are listed as below: 
\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
    \item \textit{SECOND \cite{yan2018second}:} is the first to employ the sparse convolution on the voxel-based 3D object detection task and the detection efficiency has been highly improved compared to previous work such as VoxelNet \cite{zhou2018voxelnet}. 
     \item \textit{PointPillars \cite{lang2019pointpillars}} divides the point cloud into pillars rather than voxels, and ``Pillar Feature Net'' is applied to each pillar for extracting the point feature. Then 2d convolution network is adopted on the bird-eye-view feature map for object detection. PointPillars is a trade-off between efficiency and performance.
     \item \textit{PointRCNN \cite{shi2020points}} is a pure point cloud-based two-stages 3D object detector. For extract multi-scale features, the PointNet++ \cite{qi2017pointnet++} is taken as the backbone. First, the region proposal is generated with a binary foreground/background classifier in the first stage and then the proposal is refined by cropped points and features in the second stage.
     \item\textit{PV-RCNN \cite{shi2020pv}} is a hybrid point-voxel-based 3D object detector, which can utilize the advantages from both the point and voxel representations.
\end{enumerate}

\textbf{Evaluation Results on KITTI Dataset}



\begin{table*}[ht!]
%\renewcommand\arraystretch{1.3}
\centering
 %\renewcommand\arraystretch{1.1}
\resizebox{0.75\textwidth}{!}
{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{r|c|lll|lll|lll}
\hline
\multicolumn{1}{r|}{\multirow{2}{*}{\textbf{Methods}}} &\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{mAP} (Mod)}} & %\multicolumn{1}{l|}{} &
\multicolumn{3}{c|}{\textbf{Car}} & %\multicolumn{1}{l}{} & 
\multicolumn{3}{c|}{\textbf{Pedestrian}} & 
%\multicolumn{1}{l|}{} &
\multicolumn{3}{c}{\textbf{Cyclist}}  \\ %\cline{2-14} 

{} & {} & {Easy} & {Mod.} & {Hard} & %{l}{} & 
{Easy} & {Mod.} & {Hard} & %{l|}{} & 
{Easy} & {Mod.} & {Hard}  \\ \hline  \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%{l}{} &  &  & {l|}{} & {l|}{} &  &  & {l|}{} & {l|}{} &  &  &  &  & {l|}{} \\ \hline
{Pointpillars} & {62.90} 
%& {} 
& {87.59} & {78.17} & {75.23} & %{} &
 {53.58} & {47.58} & {44.04} & %{} & 
{82.21} & {62.95} & {58.66} \\

{PointPillars$^{\star}$} & {65.78} & %{} &
{89.58} & {78.60} & {75.63} & %{} & 
{60.22} & {54.23} & {49.49} & %{} & 
84.83 & 64.50 & {60.17} \\ %\cdashline{2-14}[2pt/2pt]

{Improvement} & \RED{+2.88} & 
%{} & 
\RED{+1.99} & \RED{+0.43} & \RED{+0.4} & %{} & 
\RED{+6.64} & \RED{+6.65} & \RED{+5.45} & %{} & 
\RED{+2.62} & \RED{+1.55} & \RED{+1.51} \\ \hline

%{} &  &  & {} & {} &  &  & {} & {} &  &  &  &  &  \\ \hline

{SECOND} & {66.64} & 
%{} & 
{90.04} & {81.22} & {78.22} & %{} & 
{56.34} & {52.40} & {46.52} & %{} & 
83.94 & 66.31 & {62.37} \\
%%%%%%%%%%%%%%%%%%%%%
{SECOND$^{\star}$} & {67.17} & 
%{} & 
{91.19} & {82.13} & {79.25} & %{} &
 {56.75} & {52.80} & {48.48} & %{} & 
84.46 & 66.57 & {62.51} \\ %\cdashline{2-14}[2pt/2pt]
%%%%%%%%%%%%%%%%%%%
{Improvement} & \RED{+0.53} & 
%{} & 
\RED{+1.15} & \RED{+0.91} & \RED{+1.03} & %{} & 
\RED{+0.41} & \RED{+0.40} & \RED{+1.96} & %{} & 
\RED{+0.52} & \RED{+0.26} & \RED{+0.14} \\ \hline 

%{} &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{PointRCNN} & {69.41} & 
%{} & 
{89.68} & {80.45} & {77.91} & %{} & 
{65.60} & {56.69} & {49.92} & %{} & 
91.01 & 71.10 & {66.61} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{PointRCNN$^{\star}$} & {70.46} & 
%{} & 
{89.91} & {82.44} & {78.35} & %{} & 
{66.19} & {56.78} & {50.34} & %{} & 
94.72 & 72.16 & {67.62} \\ %\cdashline{2-14}[2pt/2pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{Improvement} & \RED{+1.05} & 
%{} & 
\RED{+0.23} & \RED{+1.99} & \RED{+0.44} & %{} & 
\RED{+0.59} & \RED{+0.09} & \RED{+0.42} & %{} & 
\RED{+3.71} & \RED{+1.06} & \RED{+1.01} \\ \hline

%{} &  &  &  &  &  &  & {} & {} &  &  &  &  &  \\ \hline

{PV-RCNN} & {71.82} &
%{} & 
{92.23} & {83.10} & {82.42} & %{} & 
{65.68} & {59.29} & {53.99} & %{} & 
91.57 & 73.06 & {69.80} \\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{PV-RCNN$^{\star}$} & {73.95} & 
%{} & 
{91.54} & {84.59} & {82.66} & %{} & 
{69.12} & {61.61} & {55.96} & %{} & 
92.82 & 75.65 & {71.03} \\ %\cdashline{2-14}[2pt/2pt]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
{Improvement} & \RED{+2.13} & 
%{} & 
\GRE{-0.69} & \RED{+1.49} & \RED{+0.24} & %{} & 
\RED{+3.44} & \RED{+2.32} & \RED{+1.97} & %{} & 
\RED{+1.25} & \RED{+2.59} & \RED{+1.23} \\ \hline
\end{tabular}
}
\label{tab:kitti_3D_detection}
\caption{\normalfont Evaluation of object 3D detection on KITTI ``val'' split for different baseline approaches. $^{\star}$ represents the baseline by adding the proposed fusion modules. }
\end{table*}




\begin{table*}[ht!]
\renewcommand\arraystretch{1.3}
\centering
 \renewcommand\arraystretch{1.1}
\resizebox{0.90\textwidth}{!}
{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{cllllllllll}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Method}} & \multicolumn{1}{c||}{mAP}  & \multicolumn{3}{c||}{Car} (AP_{70})  & \multicolumn{3}{c||}{Pedestrain} (AP_{70})  & \multicolumn{3}{c|}{Cyclist} (AP_{70}) \\ \cline{2-11} 

\multicolumn{1}{|c|}{} & \multicolumn{1}{c||}{Mod.}  & \multicolumn{1}{c|}{Easy} & \multicolumn{1}{c|}{Mod.} & \multicolumn{1}{c||}{Hard}  & \multicolumn{1}{c|}{Easy} & \multicolumn{1}{c|}{Mod.} & \multicolumn{1}{c||}{Hard}  & \multicolumn{1}{c|}{Easy} & \multicolumn{1}{c|}{Mod.} & \multicolumn{1}{c|}{Hard} \\ \hline \hline

\multicolumn{1}{|c|}{Pointpillars} & \multicolumn{1}{l||}{69.18}  & \multicolumn{1}{l|}{92.50} & \multicolumn{1}{l|}{87.80} & \multicolumn{1}{l||}{87.55}  & \multicolumn{1}{l|}{58.58} & \multicolumn{1}{l|}{52.88} & \multicolumn{1}{l||}{48.30}  & \multicolumn{1}{l|}{86.77} & \multicolumn{1}{l|}{66.87} & \multicolumn{1}{l|}{62.46} \\

\multicolumn{1}{|c|}{PointPillars(ours)} & \multicolumn{1}{l||}{72.13}  & \multicolumn{1}{l|}{94.39} & \multicolumn{1}{l|}{87.65} & \multicolumn{1}{l||}{89.86}  & \multicolumn{1}{l|}{64.84} & \multicolumn{1}{l|}{59.57} & \multicolumn{1}{l||}{55.16}  & \multicolumn{1}{l|}{89.55} & \multicolumn{1}{l|}{69.18} & \multicolumn{1}{l|}{64.65} \\
\multicolumn{1}{|c|}{\uparrow} & \multicolumn{1}{l||}{+2.95}  & \multicolumn{1}{l|}{+1.89} & \multicolumn{1}{l|}{-0.15} & \multicolumn{1}{l||}{+2.31}  & \multicolumn{1}{l|}{+6.26} & \multicolumn{1}{l|}{+6.69} & \multicolumn{1}{l||}{+6.86}  & \multicolumn{1}{l|}{+2.78} & \multicolumn{1}{l|}{+2.31} & \multicolumn{1}{l|}{+2.19} \\ \hline


\multicolumn{1}{|c|}{SECOND} & \multicolumn{1}{l||}{71.95}  & \multicolumn{1}{l|}{92.31} & \multicolumn{1}{l|}{88.99} & \multicolumn{1}{l||}{86.59}  & \multicolumn{1}{l|}{60.5} & \multicolumn{1}{l|}{56.21} & \multicolumn{1}{l||}{51.25}  & \multicolumn{1}{l|}{87.30} & \multicolumn{1}{l|}{70.65} & \multicolumn{1}{l|}{66.63} \\
\multicolumn{1}{|c|}{SECOND(Ours)} & \multicolumn{1}{l||}{73.72}  & \multicolumn{1}{l|}{94.25} & \multicolumn{1}{l|}{90.61} & \multicolumn{1}{l||}{88.19}  & \multicolumn{1}{l|}{62.37} & \multicolumn{1}{l|}{57.99} & \multicolumn{1}{l||}{54.23}  & \multicolumn{1}{l|}{89.41} & \multicolumn{1}{l|}{72.56} & \multicolumn{1}{l|}{67.38} \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{l||}{+1.77}  & \multicolumn{1}{l|}{+1.94} & \multicolumn{1}{l|}{+1.62} & \multicolumn{1}{l||}{+1.6}  & \multicolumn{1}{l|}{+1.87} & \multicolumn{1}{l|}{+1.78} & \multicolumn{1}{l||}{+2.98}  & \multicolumn{1}{l|}{+2.11} & \multicolumn{1}{l|}{+1.91} & \multicolumn{1}{l|}{+0.75} \\ \hline


\multicolumn{1}{|c|}{PointRCNN} & \multicolumn{1}{l||}{74.13}  & \multicolumn{1}{l|}{93.04} & \multicolumn{1}{l|}{88.70} & \multicolumn{1}{l||}{86.64}  & \multicolumn{1}{l|}{68.25} & \multicolumn{1}{l|}{59.41} & \multicolumn{1}{l||}{53.71}  & \multicolumn{1}{l|}{94.39} & \multicolumn{1}{l|}{74.27} & \multicolumn{1}{l|}{69.70} \\
\multicolumn{1}{|c|}{PointRCNN(ours)} & \multicolumn{1}{l||}{74.92}  & \multicolumn{1}{l|}{93.33} & \multicolumn{1}{l|}{89.13} & \multicolumn{1}{l||}{86.92}  & \multicolumn{1}{l|}{68.63} & \multicolumn{1}{l|}{59.92} & \multicolumn{1}{l||}{54.08}  & \multicolumn{1}{l|}{95.69} & \multicolumn{1}{l|}{75.70} & \multicolumn{1}{l|}{71.09} \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{l||}{+0.79}  & \multicolumn{1}{l|}{+0.29} & \multicolumn{1}{l|}{+0.43} & \multicolumn{1}{l||}{0.28}  & \multicolumn{1}{l|}{+0.38} & \multicolumn{1}{l|}{+0.51} & \multicolumn{1}{l||}{+0.37}  & \multicolumn{1}{l|}{+1.30} & \multicolumn{1}{l|}{+1.43} & \multicolumn{1}{l|}{+1.39} \\ \hline

\multicolumn{1}{|c|}{PV-RCNN} & \multicolumn{1}{l||}{76.23}  & \multicolumn{1}{l|}{94.50} & \multicolumn{1}{l|}{90.62} & \multicolumn{1}{l||}{88.53}  & \multicolumn{1}{l|}{68.67} & \multicolumn{1}{l|}{62.49} & \multicolumn{1}{l||}{58.01}  & \multicolumn{1}{l|}{92.76} & \multicolumn{1}{l|}{75.59} & \multicolumn{1}{l|}{71.06} \\
\multicolumn{1}{|c|}{PV-RCNN(ours)} & \multicolumn{1}{l||}{78.17}  & \multicolumn{1}{l|}{94.86} & \multicolumn{1}{l|}{90.87} & \multicolumn{1}{l||}{88.88}  & \multicolumn{1}{l|}{71.99} & \multicolumn{1}{l|}{64.71} & \multicolumn{1}{l||}{59.01}  & \multicolumn{1}{l|}{96.35} & \multicolumn{1}{l|}{78.93} & \multicolumn{1}{l|}{74.51} \\
\multicolumn{1}{|c|}{} & \multicolumn{1}{l||}{+1.94}  & \multicolumn{1}{l|}{+0.36} & \multicolumn{1}{l|}{+0.25} & \multicolumn{1}{l||}{+0.35}  & \multicolumn{1}{l|}{+3.32} & \multicolumn{1}{l|}{+2.22} & \multicolumn{1}{l||}{+1.00}  & \multicolumn{1}{l|}{+3.59} & \multicolumn{1}{l|}{+3.34} & \multicolumn{1}{l|}{+3.45} \\ \hline
\end{tabular}
}
\label{tab:kitti BEV detection}
\caption{\normalfont kitti BEV detection.}
\end{table*}

\textit{Performance on Baseline Methods:}

\textit{Comparison with other SOTA methods:}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Qualitative Results on KITTI Dataset}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Detectors, Dataset and Implementation Details} \label{subsec:dataset}
\subsection{Evaluation on the nuScenes Dataset} \label{subsec:nuScenes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Evaluation resulst show that fusing Lidar and image information always yields significant gains over LIDAR-only based methods,as we showed in Table,all the classes detect accuracy has improved.
\textit{Dataset:} nuScenes 3D object detection benchmark~\cite{nuscenes2019} has been employed for evaluation here, which is a large-scale dataset with a total of 1,000 scenes. For a fair comparison, the dataset has been officially divided into train, val, and testing, which includes 700 scenes (28,130 samples), 150 scenes (6019 samples), 150 scenes (6008 samples) respectively. For each video, only the key frames (every 0.5s) are annotated with 360-degree view. With a 32 lines LiDAR used by nuScenes, each frame contains about {300,000} points. For object detection task, 10 kinds of obstacles are considered including  ``car'', ``truck'', ``bicycle'' and ``pedestrian'' et al. Besides the point clouds, the corresponding RGB images are also provided for each keyframe. For each keyframe, there are 6 images that cover 360 fields-of-view.

\textit{Evaluation Metrics:} For 3D object detection, \cite{nuscenes2019} proposes mean Average Precision (mAP) and nuScenes detection score (NDS) as the main metrics. Different from the original mAP defined in \cite{everingham2010pascal}, nuScenes consider the BEV center distance with thresholds of \{0.5, 1, 2, 4\} meters, instead of the IoUs of bounding boxes. NDS is a weighted sum of mAP and other metric scores, such as average translation error (ATE) and average scale error (ASE).

\textit{Baselines:} in addition, to verify its universality,we  have implemented the proposed module on three different State-of-the-Art 3D object detectors as following,
\begin{itemize}
\item \textit{SECOND} \cite{yan2018second}, which is the first to employ the sparse convolution on the voxel-based 3D object detection task and the detection efficiency has been highly improved compared to previous work such as VoxelNet. 
\item \textit{PointPillars} \cite{lang2019pointpillars}, which divides the point cloud into pillars and ``Pillar Feature Net'' is applied to each pillar for extracting the point feature. Then 2d convolution network has been adopted on the bird-eye-view feature map for object detection. PointPillars is a trade-off between efficiency and performance. 
\item \textit{CenterPoint} \cite{yin2021center}, is the first anchor-free based 3D object detector which is very suitable for small object detection. 
\end{itemize}

\textit{Implementation Details:} HTCNet \cite{chen2019hybrid} and Cylinder3D \cite{zhou2020cylinder3d} are employed here as the 2D Segmentor and 3D Segmentor, respectively, due to their outstanding semantic segmentation ability. The 2D segmentor is pretrained on nuImages\footnote{\url{https://www.nuscenes.org/nuimages}} dataset, and the 3D segmentor is pretrained on nuScenes detection dataset while the point cloud semantic information can be generated by extracting the points inside each bounding box of the obstacles.

For Adaptive Attention Module, $m=11$, $C_1=64,C_2=128$, respectively, 
For each baseline, all the experiments share the same setting, the voxel size for SECOND, PointPillar and CenterPoint are $0.2m \times 0.2m \times 8 m$, $0.1m \times 0.1m \times0.2m$ and $0.075m \times 0.075m \times 0.075m$, respectively. We use AdamW \cite{ loshchilov2019decoupled} with max learning rate 0.001 as the optimizer. Follow \cite{nuscenes2019}, 10 previous LiDAR sweeps are stacked into the keyframe to make the point clouds more dense.

% for CeneterPoint the voxel size is $0.075m$, for  the voxel size is $0.075m$ and for PointPillar   the epoch number is 20, 

% 1. 2d segmentor, follow the original paper
% 2. 3d segmentor
% 3. data augmentation: rotation, 10 sweeps
% 4. parameters: 1).  voxel size  2). learning, batch size, epoch, lr 3). flip testing
% 5. all the exp same setting

%for \textit{2D Semantic Information},First we follow class mapping in nuScenes dataset, which maps original categories into 10 foreground categories, just same as nuScenes detection benchmark. We trained 2d SEG-net on coco dataset then fine-turned on nuImageSet. Most 3D detector on nuScenes dataset usually take current and past total 10 sweeps as point cloud input data for getting more surrounding information, so we project all point clouds (10 frames) to cameras of sample data. The details of sample and sweep data will be presented in \ref{subsec:dataset}. Finally we get painted point cloud. Experiments indicate that the semantic information is usefully for fusion modal pipeline. we directly borrow the trained HTCNet \cite{chen2019hybrid} model on NuImage \footnote{\url{https://www.nuscenes.org/nuimages }} for our 2D semantic segmentation task here. After obtaining the semantic information for each image, we project all the point clouds (including the sweeps and key-frames) into the 2D image to get the image-associated semantic information for each point. For \textit{3D semantic information}, the Cylinder 3D \cite{zhou2020cylinder3d} network is employed here for obtaining our 3D segmentation. For the original network, there are 16 classes including 10 foreground and 6 background classes. To be consistent with the 2D SEG-Net, we merge all the background classes into one class only. Finally, we can obtain the class probability for each point.

%\textit{Adaptive Attention Fusion Module:} while got both 2D pained and 3d pained point cloud we concat the semantics label with raw point $P_i$ as defined above,final each point present $P_{P_I}=\{{[x_i,y_i,z_i,r_i,t,L_{2d\_1}\in R^{11\times1},L_{3D_i}\in R^{11\times 1}}]\}_{i=1,2,3...s}$,

%\textit{Fusion Painting Framework:}

%As mentioned before, 2D images contain rich texture and detail information that provide complementary perspectives for 3D point clouds. Therefore, .  
%There was a lot of excellent Sem.seg works before,like [deeplabv3\cite{deeplabv3plus2018},PSPNet\cite{zhao2017pspnet},HTC\cite{chen2019hybrid},FCN\cite{shelhamer2017fully},MobelNetV3\cite{Howard_2019_ICCV}],we finally adopt HTC as our 2D image semantic segmentation modal,Specially a LIDAR  correspond to six cameras on nuScenes dataset, and there has no 2d semantic annotations with relation image,luckly nuImages is available released by same source of nuScenes dataset,so we first trained Sem.seg modal on nuImage dataset,and do inference on all sample cameras images data of nuScenes dataset,we obtain the probability of semantic classes or label index for each pixel in 2d image,because we can't get sweeps camera data with relation sample cameras ,
%{\color{red}{ADD SOME DETAILED OPERATIONS}}
%for 2D SEG-Net,we follow class mapping in nuScenes dataset, which maps original categories into 10 foreground categories [car, truck, construction\_vehicle, bus, trailer, barrier, motorcycle, bicycle, pedestrian, traffic\_cone], just same as nuScenes detection benchmark,and we first trained 2d SEG-net on ImageSet,then the detector is pre-trained on COCO train2017 dataset with 20 epochs,finally trained 20 epochs on nuImage dataset,and got 46.4 mask AP,in order to save datastore we save the result as mask image which convert the segmentation scores to label index with the highest score each pixel.because nuScenes dataset adpot 32 channels lidar,so  Most 3D detector on nuScenes dataset usually take current and past total 10 sweeps as point cloud input data for get more surrounding information,we can't find relation cameras with past sweep,for this reason,we project all points cloud on six cameras of each sample data,experiments proved that the method works,we finally convert mask image label index to one hot encoding,change the label index 1$\rightarrow11$,10 foreground class and one background.
%For 3D SEG-Net.There are 23 foreground categories annotated in nuScenes-lidarseg dataset,First of all,we mapping the categories into 10 foreground categories like 2D SEG-Net,and there also has 9 background,in 3D object detection task,we need merge them into one classes,then trained 20 epochs on nuScenes lidar-seg dataset with Cylinder modal,each point will get 11 scores vector which present 10 foreground class and one background probabilities,because there has no released evaluation code for lidar segmentation,so we test it on validation dataset and got similar results as Cylinder 3D,nuScenes LIDAR-seg dataset is same cognate as nuScene lidar data,the next,we directly inference nuScenes lidar points cloud with Cylinder pre-trained modal to save each point cloud labels,each point has it label index with highest score,finally we convert it to one hot encoding,we will concatenate 10 sweeps raw point cloud with relation labels before feed the data to the 3D detector.
 %For self-attention module:TODo


\begin{table*}[ht!]
%\renewcommand\arraystretch{1.3}
\centering
% \renewcommand\arraystretch{1.1}
\resizebox{0.95\textwidth}{!}
{
	\begin{tabular}{l | c | c | c c c c c c c c c c}
	\hline
    \multicolumn{1}{c|}{\multirow{2}{*}{Methods}} &
    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{NDS}(\%)}} &
    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{mAP}(\%)}} & 
    \multicolumn{10}{c}{\textbf{AP} (\%)} \\
    
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l}{Car} & \multicolumn{1}{l}{Pedestrian} & \multicolumn{1}{l}{Bus} & \multicolumn{1}{l}{Barrier} & \multicolumn{1}{l}{T.C.} &
    \multicolumn{1}{l}{Truck} & \multicolumn{1}{l}{Trailer} & \multicolumn{1}{l}{Moto.} & \multicolumn{1}{l}{Cons.} &
    \multicolumn{1}{l}{Bicycle} \\ 
    \hline \hline
    %\multicolumn{1}{l}{mAP} & \multicolumn{1}{l}{Car} & \multicolumn{1}{l}{Pedestrian} & \\
    %\textbf{Methods} & NDS & mAP & Car & Pedestrian & Bus & Barrier & T.C. & Truck & Trailer & Moto. & Cons. & Bicycle &  \hline
	

	SECOND \cite{yan2018second}  &61.96 &50.85 &81.61  &77.37 & 68.53 &57.75  &56.86  &51.93 &38.19 & 40.14 &17.95 & 18.16 \\
	SECOND$^{\ast}$ & 67.41  & 62.15  & 83.98  & 82.86 &71.13 &63.29 &74.66 &59.97 &41.53 &66.85 &22.90  &54.35  \\
	Improvement $\uparrow$ & \textcolor{red}{{+5.45}} & \textcolor{red}{{+11.30}} & \textcolor{red}{+2.37} & \textcolor{red}{+5.49} & \textcolor{red}{+2.60} & \textcolor{red}{+5.54} & \textcolor{red}{+17.80} & \textcolor{red}{+8.04} & \textcolor{red}{+3.34} & \textcolor{red}{+26.71} & \textcolor{red}{+5.05}& \textcolor{red}{+36.19} \\
    \hline
	
	PointPillars \cite{lang2019pointpillars}  & 57.50 &43.46 &80.67 &70.80 &62.01 &49.23 &44.00 &49.35 &34.86 &26.74 &11.64 &5.27 \\
	PointPillars$^{\ast}$ &66.04 & 60.77&83.51 &82.90&69.96 &58.46&74.50&56.90&39.25&66.40&21.68&54.10   \\
	Improvement $\uparrow$ & \textcolor{red} {{+8.54}} & \textcolor{red}{{+17.31}} & 
	\textcolor{red}{+2.84} & \textcolor{red}{+12.10} & \textcolor{red}{+7.95 } & \textcolor{red}{ +9.23} & \textcolor{red}{+30.50} & \textcolor{red}{+7.55} & \textcolor{red}{+4.39} & \textcolor{red}{+39.66}  & \textcolor{red}{+10.04} & \textcolor{red}{+48.83} \\
    \hline
	
	CenterPoint \cite{yin2021center}  & 64.82 &56.53 &84.73 &83.42 &66.95 &64.56 &64.76 &54.52 &36.13 &56.81 &15.81 &37.57\\
	CenterPoint$^{\ast}$ &70.68 &66.53 &87.04 &88.44 & 70.66 &67.26 &79.57 &62.98 & 45.09 & 74.65&25.36&64.41\\
	Improvement $\uparrow$ & \textcolor{red}{\textbf{+5.86}} & \textcolor{red}{\textbf{+10.00}} & \textcolor{red}{+2.31} & \textcolor{red}{+5.02} & \textcolor{red}{+3.71} & \textcolor{red}{+2.70} & \textcolor{red}{+14.81} & \textcolor{red}{+8.46} & \textcolor{red}{+8.96} & \textcolor{red}{+17.84} &  \textcolor{red}{+9.55}&\textcolor{red}{+26.84} \\
    \hline
	\end{tabular}
}
\caption{\normalfont Evaluation results on nuScenes validation dataset. ``NDS'' and ``mAP'' mean nuScenes detection score and mean Average Precision. ``T.C.'', ``Moto.'' and ``Cons.'' are short for ``traffic cone'', ``motorcycle'', and ``construction vehicle'' respectively. `` * '' denotes the improved baseline by adding the proposed ``FusionPainting''. To hight the effectiveness of our methods, the improvements of each method are demonstrated in red.}
\label{tab:eval_on_nuscenes_val}
\end{table*}







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Evaluation Results on nuScenes Dataset} \label{subsubsec:evaluation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We have evaluated the proposed framework on nuScenes benchmark for both validation and test splits.

\textit{Performance on Baseline Methods:} First of all, we have integrated the proposed fusion module into three different baselines methods and experimentally we have achieved consistently improvements on both $\text{mAP}$ and $\text{NDS}$ compared to all baselines. Detailed results are given in Tab. \ref{tab:eval_on_nuscenes_val}. From this table, we can obviously find that the proposed module gives more than 10 points improvements on $\text{mAP}$ and  5 points improvements on $\text{NDS}$ for all the three baselines. The improvements have reached 17.31 and 8.45 points for PointPillars method  on $\text{mAP}$ and $\text{NDS}$ respectively. In addition, we find that the ``Traffic Cone'', ``Moto'' and ``Bicycle'' have received the surprising improvements compared to other classes. For ``Bicycle'' category specifically, the AP has improved about \textbf{36.19\%}, \textbf{48.83\%} and \textbf{26.84\%} based on Second, PointPillar and Centerpoint respectively. Interestingly, all these categories are small objects which are hard to be detected because of a few LiDAR points on them. By adding the prior semantic information, the category classification becomes relatively easier. Especially, the experiments here we share the same setting, so the baseline figures may be subtle differences with official.

%For example, the AP of ``Bicycle'' based on Second, PointPillar and Centerpoint has improved \textbf{+36.19}, \textbf{+48.83} and \textbf{+26.84} respectively,
%Evaluation result show that fusing Lidar and image information always yields significant gains over LIDAR-only based methods,as we showed in Tab. \ref{tab:eval_on_nuscenes}, all the classes detect accuracy has surprising improved,for both PointPillars,Second and CenterPoint detector,the Bicycle class received the Traffic Cone,Moto and Bicycle reveived *,*,* (AP)increased,and for Both  PointPillar , Traffic Cone,Moto and Bicycle AP received *,*,* increased,The reason,I think is that there has few point on such categories because sparse 3D points characteristic of LIDAR,So,it need extra information to identify the real class.
\textit{Comparison with other SOTA methods:} To compare the proposed framework with other SOTA methods, we submit our best results (proposed module on the CenterPoint \cite{yin2021center}) to the nuScenes evaluation sever\footnote{\url{https://www.nuscenes.org/object-detection/}}. The detailed results are listed in Tab. \ref{tab:test_tabel}. To be clear, only these methods with publications are compared here due to space limitation. From this table, we can find that the ``NDS'' and ``mAP'' have been improved by 3.1 points and 6.0 points respectively compared with the baseline method CenterPoint \cite{yin2021center}. More importantly, our algorithm outperforms previous multi-modal method 3DCVF \cite{DBLP:conf/eccv/YooKKC20} by a large margin, \textit{i.e.}, improving 8.1 and 13.6 points in terms of NDS and mAP metrics.
%finally compare our method with previous state-of-the-art 3D objection methods on nuScenes Leaderboard,which ranked top five with LIDAR only and combine LIDAR and Camera methods respectively,the result as showed in Tabel.\ref{tab:test_tabel},
\begin{figure*}[ht!]
	\centering
	\includegraphics[width=0.975\textwidth]{FusionPainting/TITS/Figs/results_rviz.pdf}
	\centering
	\caption{Visualization of detection results, where (a) is the ground-truth, (b) is the detection results based on raw point cloud, (c), (d) and (e) are the detection results based on the projected points with 2D semantic information, 3D semantic information and fusion semantic information, respectively. Especially, the yellow and red dash ellipses show some of the false and missed detection, respectively. The baseline detector used here is CenterPoint.} %	A is Ground trues/raw point and corresponding image, B and C are the projected point with 3d and 2D semantic information respectively,D is the results of our method.Vehicles are showed in red 
	\label{Fig:detection result}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Qualitative Results on nuScenes Dataset}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

More qualitative detection results are illustrated in Fig. \ref{Fig:detection result}. Fig. \ref{Fig:detection result} (a) shows the annotated ground truth, (b) is the detection results for CenterPoint based on raw point cloud without using any painting strategy. (c) and (d) show the detection results with 2D painted and 3D painted point clouds, respectively, while (e) is the results based on our proposed framework. 
As shown in the figure, there are false positive detection results caused 2D painting due to frustum blurring effect, while 3D painting method produces worse foreground class segmentation compared to  2D image segmentation.  Instead, our FusionPainting can combine two complementary information from 2D and 3D segmentation, and detect objects more accurately.

% The advantage of FusionPainting is obvious, the 2D painting brings more false positive, caused by the frustum blurring effect, while 3D painting gives worse foreground class detect compared to the 2D image semantic as we discussed above, The FusionPainting proven the great advantages of combining two complementary information and made the results more accurate. 


      
\begin{table*}[ht!]
    \centering
    \renewcommand\arraystretch{1.2}
\resizebox{0.95\textwidth}{!}{

\begin{tabular}{ l| c| c| c| c c c c c c c c c c}
    \hline
    \multicolumn{1}{c|}{\multirow{2}{*}{Methods}}  & 
    \multicolumn{1}{c|}{\multirow{2}{*}{Modality}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{NDS}(\%)}} & 
    \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{mAP}(\%)}} & 
    \multicolumn{10}{c}{\textbf{AP} (\%)} \\ 
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & \multicolumn{1}{l}{Car} & \multicolumn{1}{l}{Truck} & \multicolumn{1}{l}{Bus} & \multicolumn{1}{l}{Trailer} & \multicolumn{1}{l}{Cons} & \multicolumn{1}{l}{Ped} & \multicolumn{1}{l}{Moto} & \multicolumn{1}{l}{Bicycle} & \multicolumn{1}{l}{T.C} & \multicolumn{1}{l}{Barrier} \\ \hline
    PointPillars \cite{vora2020pointpainting} & L & 55.0 & 40.1 & 76.0 & 31.0 & 32.1 & 36.6 & 11.3 & 64.0 & 34.2 & 14.0 & 45.6 & 56.4 \\
    3DSSD \cite{yang20203dssd} & L  & 56.4 & 46.2 & 81.2  & 47.2  & 61.4  &  30.5 & 12.6 &  70.2 & 36.0  &  8.6 &  31.1 &  47.9 \\
    
    CBGS \cite{zhu2019class} & L & 63.3 & 52.8 & 81.1 & 48.5 & 54.9 & 42.9 & 10.5 & 80.1 & 51.5 & 22.3 & 70.9 & 65.7 \\
    %CyliNET \fangjin{no paper}& L & 66.1 & \multicolumn{1}{c}{58.5} & 85.0 & 50.2 & 56.9 & 52.6 & 19.1 & 84.3 & 58.6 & 29.8 & 79.1 & 69 \\
    HotSpotNet \cite{chen2020object} & L & 66.0 & 59.3 & 83.1  & 50.9 & 56.4  & 53.3  &  {23.0} &  81.3 & {63.5}  &  36.6 &  73.0 &  \textbf{71.6} \\
    CVCNET\cite{chen2020every} & L & 66.6 & 58.2 & 82.6 & 49.5 & 59.4 & 51.1 & 16.2 & {83.0} & 61.8 & {38.8} & 69.7 & 69.7 \\
    CenterPoint \cite{yin2021center} & L & {67.3} & {60.3} & {85.2} & {53.5} & {63.6} & {56.0} & 20.0 & 54.6 & 59.5 & 30.7 & ne{78.4} & 71.1 \\
    PointPainting \cite{vora2020pointpainting} & L \& C & 58.1 & 46.4 & 77.9 & 35.8 & 36.2 & 37.3 & 15.8 & 73.3 & 41.5 & 24.1 & 62.4 & 60.2 \\
    3DCVF \cite{DBLP:conf/eccv/YooKKC20} & L \& C & 62.3 & 52.7 & 83.0 & 45.0 & 48.8 & 49.6 & 15.9 & 74.2 & 51.2 & 30.4 & 62.9 & 65.9 \\ \hline
    %MOCA & L \& C & 70.9 & \multicolumn{1}{c}{66.6} & 86.7 & 58.6 & 67.2 & 60.3 & 32.6 & 87.1 & 67.8 & 52 & 81.3 & 72.3 \\
    %PointAugmenting & L \& C & 71.1 & \multicolumn{1}{c}{66.8} & 87.5 & 57.3 & 65.2 & 60.7 & 28 & 87.9 & 74.3 & 50.9 & 83.6 & 72.6 \\ 
    {FusionPainting(Ours)} & L \& C & \textbf{70.4} & \textbf{66.3} & \textbf{86.3} & \textbf{58.5} & \textbf{66.8} & \textbf{59.4} & \textbf{27.7} & \textbf{87.5} & \textbf{71.2} & \textbf{51.7} & \textbf{84.2} & {70.2}  \\  \hline
    % {Improvement$\uparrow$} &  & \textcolor{red}{\textbf{+3.1}} &  \textcolor{red}{\textbf{+6.0}} & \textcolor{red}{\textbf{+1.1}& \textcolor{red}{\textbf{+5.0}}} & \textcolor{red}{\textbf{+3.2}} & \textcolor{red}{\textbf{+3.4}} & \textcolor{red}{\textbf{+4.7}} & \textcolor{red}{\textbf{+4.5}} & \textcolor{red}{\textbf{+7.7}} & \textcolor{red}{\textbf{+12.9}} & \textcolor{red}{\textbf{+5.8}} & {-1.4} \\ \hline
    \end{tabular}
}
\caption{Comparison with other SOTA methods on the nuScenes 3D object detection benchmark. ``L'' and ``C'' in the modality column represent lidar and camera respectively. For each column, we use ``underline'' to illustrate the best results of other methods and we give the improvements of our method compared to other best performance. Here, we only list all the methods results with publications.}
\label{tab:test_tabel}
\end{table*}
